Aiding Humans in Financial Fraud Decision Making: Toward an XAI-Visualization Framework

AI prevails in financial fraud detection and decision making. Yet, due to concerns about biased automated decision making or profiling, regulations mandate that final decisions are made by humans. Financial fraud investigators face the challenge of manually synthesizing vast amounts of unstructured information, including AI alerts, transaction histories, social media insights, and governmental laws. Current Visual Analytics (VA) systems primarily support isolated aspects of this process, such as explaining binary AI alerts and visualizing transaction patterns, thus adding yet another layer of information to the overall complexity. In this work, we propose a framework where the VA system supports decision makers throughout all stages of financial fraud investigation, including data collection, information synthesis, and human criteria iteration. We illustrate how VA can claim a central role in AI-aided decision making, ensuring that human judgment remains in control while minimizing potential biases and labor-intensive tasks.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016
modified by Matt Brehmer, Feb 2024

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE VIS: Visualization & Visual Analytics (Short Papers, Posters)
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> oldRelatedWorktext.tex <==
\section{Borrow from Old Text: Thesis random copy}

The United Nations Office on Drugs and Crime (UNODC) estimates that each year, roughly 2 to 5 percent of the global GDP, equivalent to between EUR 715 billion and 1.87 trillion, is involved in money laundering \cite{europol}. The sources of these illegal funds range from activities like drug trafficking, human trafficking, child pornography, and extortion. In addition, the Netherlands ranks as the eighth most attractive country for money launderers among the top ten global destinations, according to Dutch bank associations \cite{nvb}. Despite these alarming statistics, the government report suggests that larger banks and financial institutions tend to classify a disproportionate number of customers as low risk without proper justification \cite{financien_anti-money_2022}. This raises concerns about their Anti Money Laundering (AML) investigation processes, highlighting the urgent need for financial organizations to clarify their decision making processes and substantiate their rationale for marking certain customers as low risk.

By conducting a systematic literature review, \cite{al-suwaidi_anti-money_2020}'s work provides a comprehensive survey of previous AML research. More importantly, the paper sets a list of agenda for future research. It advocates for detecting schemes using machine learning and leveraging the power of artificial intelligence systems to identify potential money laundering and terrorist financing accounts. 

The adoption of machine learning has proven to be an effective tool against financial crimes, overcoming the limitations of rule-based systems. Since rule-based models lack learning and generalization capabilities to adapt to unknown patterns \cite{Gao_Xu}, machine learning systems enhance the efficacy of computer algorithms by learning from a variety of resources \cite{Bayramoğlu} \cite{Chao_et_al}. Based on the algorithmic patterns that the machine learning system learned from input data, the system can make predictions or decisions about new data. Some common machine learning techniques being used to fight financial crime are data mining, behavior analysis and graph computing \cite{Chao_et_al} \cite{Gao_Ye} \cite{Goecks} \cite{Kurshan_Shen} \cite{Rao_Kanchana} \cite{Velasco}. However, there are technical complexities associated with machine learning, such as accuracy in alert detection, difficulty in acquiring labeled data, data quality. In addition, machine learning also suffer from "human out of the loop" design and machine learning intepretability (see section \ref{MLchallenges}).

To address the "human out of the loop" design and machine learning intepretability, \cite{Singh_Best} proposed to use visualization to leverage AML investigation. According to \cite{Singh_Best}, previous research in AML has largely focused on combating money laundering, implementing regulations, and using technology to monitor suspicious activity. However, their study aimed to fill a knowledge gap by demonstrating how visualization of monetary transactions can effectively detect money laundering. Their research showed that visualization can be a powerful tool for identifying suspicious behavior patterns, and can help investigators target these behaviors more efficiently. By using data visualization techniques, 

's study suggests that investigators can improve their ability to detect and prevent money laundering.

The role of visualization in AML investigations is crucial, however, this study aims to go beyond that by bringing clarity to the often opaque decision making procedures within financial organizations. Specifically, the research seeks to shed light on the rationale behind classifying certain alerts as low risk in AML investigations. To achieve this, the study takes inspiration from Herbert \cite{Simon}'s work on decision making, which comprises three fundamental activities: Intelligence, Design, and Choice. \textit{Intelligence} refers to the problem identification process, which is carried out by gathering information that may impact the decision. After a decision maker gathers insights about the problem, he/she can evaluate the potential solutions in the \textit{Design} process. The \textit{Design} process is followed by \textit{Choice}, in which the decision maker judge between solutions and select the best solution based on a set of criteria. Through this framework, the study aims to explore and analyze decision making within the realm of AML investigations.

Although one of the ultimate goals of information visualization is to support decision making, current Information Visualization (InfoVis) studies often prioritize supporting the data analysis tasks \cite{Dimara_Stasko} \cite{Dimara2021Unmet}. However, many visualization task taxonomies fail to provide assistance on studying human decisions in the context of data analysis and visualization. This is especially true in the AML context, where studies often do not differentiate between decision makers and data analysts (see section \ref{whyinfovis}). Moreover, there is a lack of evaluation studies in InfoVis research that target decision makers as the end users \cite{Dimara_Stasko} \cite{Dimara2021Unmet}. To address these gaps, further research within AML domain should focus on evaluation studies targeting decision makers. 

Lastly, previous research did not make use of using constructive visualization to increase flexibility in decision making within AML domain. \cite{Dimara2021Unmet} recommended four types of visualization tools to support decision makers: \textit{flexible interface}, \textit{interrogator tools}, \textit{scenario-based simulations}, and \textit{trade-off overviews}. Specifically within flexible interface, the system created could make use of four approaches to improve the flexibility, including \textit{social actions}, \textit{input data actions}, \textit{mapping and presentation actions}, \textit{processing} and \textit{interaction mean} \cite{Dimara2021Unmet}. To increase the flexible of the information visualization, \cite{constructive} introduced the use of constructive visualization. Constructive visualization as the act of \textit{"constructing a visualization by assembling blocks, that have previously been assigned a data unit through a mapping"} \cite{constructive}. Constructive visualization is a novel approach that empowers individuals non-expert in data visualization to create visual representations that they can use to directly engage with datasets. This approach allows novice users to develop flexible visualizations and open up new possibilities for engaging with data \cite{constructive}. Therefore, this research aims to explore this direction and examine the effectiveness of constructive visualization in decision making during AML investigations. 

Taken together, the goal of the present study is to identify how visualizations can be embedded in the Anti Money laundering domain to improve decision making process. As a result, the following research question was formulated:

\textbf{Research question}: How can information visualization be employed to enhance the decision making process for Anti Money laundering in financial organization?

The remainder of this thesis is structured as follows. Section \ref{related-work} reviews existing research in AML, decision making, and visualization to identify research gaps. Section \ref{Methodology} outlines the research design and methodologies employed for data collection and analysis. Sections 4 through 7 detail the multi-step methodology: discover, define, develop, and deliver. These sections outline the procedure for each step of the methodology and the result of these steps. In particular, section \ref{section-discover} discuss the steps taken to discover the visualization needs for AML investigation by conducting discovery research within a real-world financial organization. Section \ref{section-define} defines design challenges based on the insights obtained during the discovery phase. Section \ref{section-develop} presents collaborative solutions developed in a Creative Problem Solving workshop. Section \ref{section-deliver} assesses the usability of the solution with AML investigators. Section \ref{section-discussion} interprets findings, comparing them with existing literature and drawing design implications. Finally, Section \ref{section-conclusion} underscores the research's significance and potential impact in enhancing AML decision making through information visualization.

\subsection{RELATED WORK}\label{related-work}
% \evanthia{add a section outline: what we will learn in this section and subsections and shortly why (i.e. are you going to use them somehow in your thesis? motivate why your reader needs to read those?}
In this section, we will explore the existing body of research and related work that informs our study. By reviewing prior studies in the field of Anti Money laundering (AML), information visualization and decision making, we aim to build upon and extend the current knowledge base. 

\subsection{Anti Money laundering: An overview}
% \evanthia{add a subsection outline: what we will learn in this section and subsubsections and very shortly why}
This section focuses on the fundamental concepts behind Anti Money laundering. By examining topics such as money laundering stages, the roles of financial organizations in combating money laundering and the regulatory framework for AML, we will gain a comprehensive understanding of the complexities involved in combating financial crimes.

\subsubsection{What is money laundering?}\hfill\\
This section will delve into the fundamental concepts behind money laundering by presenting the definition of money laundering and the process it entails. 

\textit{Money laundering} is defined as the process of carrying out illegal activities to make illegally obtained funds appear legal and legitimate \cite{Goecks}, \cite{Zhou}. Some key illegal activities include organized crime, drug trafficking, and terrorist financing \cite{Cox}. In a broader sense, money laundering could also be a cover-up for other criminal activities, such as robbery, theft, extortion, corruption, and tax evasion. 

The process of money laundering usually entails three steps: \textit{placement, layering, and integration}. \textit{Placement} refers to the process of making the money at its source appear different by breaking it up into smaller amounts \cite{Goecks}. There are some businesses where the risk for money laundering to take place is higher, such as launderettes, newspaper sales, restaurants, casinos, insurance, asset management, antiques, and property \cite{Cox}. Meanwhile, \textit{layering} aims to hide the washing activities and bypass  detection through a sequence of conversions. Laundered funds are then \textit{integrated} back into the economy, mostly through the financial institutions, giving the impression that they are regular business gains \cite{Cox}.

\subsubsection{Why do financial organizations need to fight against money laundering?}\hfill\\
Since financial organizations could be exploited by money launderers to integrate illicit funds back to the economy, there are several reasons why financial organizations need to adopt extra precautions. This section explain the risks that financial organizations might face without sufficient anti money laundering measures.

Financial institutions, such as banks, FinTech companies, investment firms, and insurance providers play a vital role in the fight against money laundering since they can be involved in financial crime as a victim, an instrumentality, or even a perpetrator of money laundering activities \cite{Kurshan_Shen}. As money laundering techniques are becoming more complex with the rise of digital technologies, financial institutions need to comply with legal requirements to ensure the integrity of their financial systems. 
A financial institution may face several risks if they do not provide adequate anti money laundering, including \textit{operational risk, regulatory risk, and reputational risk} \cite{Cox}. 

\textit{Operational risk} refers to the loss resulting from internal failures of the organization, particularly people, processes, and systems. For example, this type of risk occurs when a financial company fails to perform a customer background check or inadequately reports to authorities. As a consequence of failing to meet AML compliance, the company may face penalties from the authorities. 

\textit{Regulatory risk} is a subset of operational risk, which require a financial company to have sufficient policies and procedures to comply with local and international regulations. The responsibility to handle regulatory risk often belongs to the money laundering reporting officer, who is in charge of monitoring high-risk customers and suspicious activities, conducting regular risk assessments, and reporting financial crimes. Employee training is an essential step to mitigate  both regulatory and operational risks. 

\textit{Reputational risk} is the last type of risk usually associated with money laundering. Negative publicity resulting from money laundering incidents can damage a  financial institution's brand value, leading to a loss of customers and revenue \cite{Cox}. Therefore, financial organizations must fight against money laundering, not only to comply with regulations but also to safeguard their customers and avoid reputational damage. 

\subsubsection{What are the standard procedures in Anti Money Laundering?}\hfill\\
In this section, we introduce the Anti Money Laundering regulatory framework and outline the necessary measures that financial organizations must undertake to combat money laundering. 

\textit{Anti Money Laundering (AML)} refers to a set of laws, regulations, and standards with the aim at counteracting money laundering \cite{Tsingou}. Financial institutions need to perform multiple standard procedures to comply with AML regulations, such as \textit{Customer Due Diligence, Transaction Monitoring, Suspicious Activity Reporting} \cite{Cox}.

\textbf{Customer Due Diligence}\hfill\\ 
Financial institutions are required to perform customer due diligence, which refers to the procedure of identifying their customers and associates \cite{Cox}. This due diligence procedure aims to ensure that the customers and associates have a legitimate source of funds and they do not pose any risks to both the company and society. While Customer Due Diligence emphasizes evaluating the customer risk profile, \textit{Know Your Customer (KYC)} is a part of Customer Due Diligence that focuses on identity verification. KYC is the process conducted by financial companies to perform background checks when new clients and customers are onboard. The result of the KYC process will determine whether a company should establish a relationship with this customer or not. Accordingly, if a financial company has a suspicion about the customer's identity, this customer should not be allowed to continue using the company’s financial services \cite{Cox}. 

\textbf{Transaction Monitoring}\hfill\\ \label{AMLworkflow}
Even after the customer's identity is verified, financial institutions still need to monitor the customer's activities in the financial system to make sure that the customer does not abuse the system for illegal activities. Transaction monitoring refers to the process of identifying suspicious patterns within  transactions and warranting further investigation  . Monitoring involves investigating the transactions to make sure the transactions are consistent with the company’s existing information obtained from the Customer Due Diligence.

In some cases, more intensive monitoring is required when the financial organizations need to take a deeper dive into the analysis and perform further due diligence. This process refers to \textit{Enhanced Ongoing Monitoring} \cite{Sullivan}. This enhanced process can be triggered by various factors, including the type of transactions, customer profile, the parties concerned, comparison with similar customers, geographical area, and product risk \cite{Sullivan}. If a target requires further monitoring, the financial institutions will take additional measures, such as getting more detailed data about the customer's job or source of funds, performing periodic reviews of the customer's transactions, or assigning a transaction monitoring analyst to watch the customer's activities \cite{Cox}.

In a traditional pipeline of AML transaction monitoring investigation, there are four layers of investigation: \textit{Data}; \textit{Screening and Monitoring}; \textit{Alert and Event}; and \textit{Operational Layer}. In the \textit{Data} layer, the system collects and handles internal data sourced from financial institutions, as well as external data obtained from regulatory agencies, authorities, and watch lists \cite{Han_et_al_2}. The second layer, \textit{Screening and Monitoring}, checks on transactions and clients to identify any suspicious activity, which is often automated (see section \ref{machinelearning}). If a suspicious activity needs to be reviewed by a human investigator, an alert would be raised in the \textit{Alert and Event} for further investigation. To provide a thorough examination of the flagged transaction, this stage entails supplementing the data with past transaction information and relevant evidence. Based on the information obtained from the previous stages, human agents make the ultimate decision whether to block, release, or queue a transaction in the \textit{Operational Layer}. Financial organizations are legally obligated to have a human agent must make the ultimate determination regarding a transaction \cite{Han_et_al_2}.

\textbf{Suspicious Activity Reporting}\hfill\\ \label{SAR}
Reporting unusual and suspicious activities is essential for financial institutions to comply with regulatory requirements \cite{Cox}. There are several indications of suspicious activity, such as customer activity that is inconsistent with the company’s understanding of this customer, a customer who opens several accounts with high transaction frequency, or an account with little to no activity that seems to be a temporary repository for funds to be transferred abroad.
\cite{Zhou} categorized the transaction behaviors into loud and subtle activity. The loud tactic involves performing high frequency transaction or high-volume transaction, which is easier to detect. The subtle tactic is more challenging to detect since the criminals disguise themselves as regular accounts and perform transactions in regular frequency and volume. 
However, many other activities could also be indicative of money laundering, such as an ambiguous source of income, frequent address changes, negative media reports, or transfers of company funds to private accounts. Since there are multiple factors that need to be considered when reporting suspicious activity, the authorities require reporting procedure to have clear audit trails that document the actions and decisions being undertaken by the financial organizations \cite{Cox}.

\subsection{The use of Machine Learning in AML} \label{machinelearning}
% \evanthia{add a subsection outline e.g., Am I gonna need to understnad/use behavior analysis, data mining, graph drawing? }
In order to improve the current implementation of AML applications, it is important to understand how money laundering is being detected. The following section provides more details on the machine learning techniques are being used to support AML and their current challenges.  

\subsubsection{How are the AML procedure supported by Machine Learning methods?}\hfill\\
Traditional anti money laundering systems usually make use of complex rules and thresholds to spot suspicious patterns and generate alerts. However, there are several challenges with a rule-based system:
\begin{enumerate}
\item The rule-based systems often result in a high number of false positive alerts \cite{Han_et_al_2}.
\item A rule-based AML strategy also won't be able to respond to changes in criminal conduct that are that seek to conceal it from authorities \cite{Mohammed}.
\item The operational burden is heavy to keep the rules up-to-date and relevant at all time \cite{jullum_detecting_2020}.
\end{enumerate}

As a result, \textit{machine learning} is widely used in AML to addresses the weaknesses of rule-based systems. Since rule-based models lack learning and generalization capabilities to adapt to unknown patterns \cite{Gao_Xu}, machine learning systems enhance the efficacy of computer algorithms by learning from a variety of resources, including data uploaded into the system, the differences between false and corrective behavior, and the measurement systems developed to guide the computer \cite{Bayramoğlu} \cite{Chao_et_al}. Based on the algorithmic patterns that the machine learning system learned from input data, the system can make predictions or decisions about new data. 

% Machine learning systems have multiple applications within the financial domain, such as classifying transactions with high accuracy, clustering transactions based on similarities and identifying complex patterns \cite{Chen_et_al.}. 

Machine learning algorithms are typically classified into two main categories: supervised and unsupervised techniques \cite{Chen_et_al.}. Supervised learning learns from a predetermined set of labeled training data, and the labels are represented as binary variables. Using this labeled training set, a supervised learning model is constructed to classify new, unseen data into different label categories. For example, supervised machine learning can be used to classify normal and suspicious transactions based on variations in credit amounts, debit amounts, credit frequency, and debit frequency \cite{Chen_et_al.}. 

Different from supervised learning, the label information is disregarded during the learning process. Unsupervised algorithms separate training data into multiple distinct groups or clusters based on their similarity to other instances within the same cluster \cite{Chen_et_al.}. In the context of AML, clustering techniques may reveal a group of often recurring, small-value transactions involving several accounts that have similar patterns of frequency. This might be an indication of criminals deliberately maintain transaction amounts below a certain level in order to avoid being noticed. By identifying such clusters, financial institutions can raise an alert on such clusters for further investigation and perhaps report them to the authorities. 

Alternatively, there are several machine learning techniques being used to fight financial crime, with \textit{data mining}, \textit{behavior analysis} and \textit{graph computing} being some of the most popular methods \cite{Goecks}.

\textit{Behavior analysis} refers to the process of user behavior identification, such as analyzing textual data within digital transactions and characterizing transactions based on user behavior \cite{Goecks}. Behavior analysis is commonly used by financial institutions to monitor and detect suspicious transactions. As a result, this method is particularly useful for \textit{Transaction Monitoring} and \textit{Suspicious Activity Reporting}. Financial organizations can use behavior analysis to identify complex transactional patterns, for example when there is a network of accounts involved in a money-laundering scam. \cite{Rao_Kanchana} employ behavior analysis to characterize user transactions and identify the connection between different accounts. The algorithm identifies large cash withdrawals from previously inactive accounts or from accounts that have recently received large deposits. The system then find additional accounts that are linked to these accounts. Based on the analysis, financial organizations can detect suspicious activities and report them to authorities. 

\textit{Data mining} is the process of using algorithms to discover information hidden in large datasets \cite{Chao_et_al}. This technique can be used in all three AML procedures (\textit{Customer Due Diligence}, \textit{Transaction Monitoring} and \textit{Suspicious Activity Reporting}) since it is effective in reducing data preparation time and false positive alerts \cite{Gao_Ye}. Financial institutions can employ data mining techniques for decision support, financial risk prevention and hidden risk model simulation \cite{Chao_et_al}. For instance, \cite{Velasco} made use of data mining algorithms to identify the corruption risk patterns within Brazilian public spending data of 50 billion dollars. Some risk patterns included collusion between bidders, conflicts of interest, and companies owned by a potentially straw person used for disguising its real owner \cite{Velasco}. This system has proven to be effective in detecting these risk patterns and provided valuable inputs for several investigations \cite{Velasco}. 

\textit{Graph computing} is used to analyze and represent complex datasets in the form of network graphs using machine learning algorithms \cite{Chao_et_al}. A graph often consists of two main components: nodes and edges. In the financial domain, nodes usually represent financial entities such as companies, individuals, accounts, locations, devices, while edges represent the transfers of funds or relationship strengths between entities \cite{Kurshan_Shen}. Graph computing can be used in AML application to discover hidden suspicious accounts by level-by-level mining of the relationships between different accounts. \cite{Chao_et_al}. Since graph computing can reveal hidden transaction patterns, identify networks of related account, it can aid AML investigators with \textit{Transaction Monitoring} and \textit{Suspicious Activity Reporting}.

\subsubsection{What are the challenges of existing Machine Learning methods?}\hfill\\ \label{MLchallenges}
The following section addresses the limitations associated with existing machine learning techniques, which highlights the necessity for financial organizations to adopt a new solution that enhances the decision making process in AML investigations. 

\textbf{Alert detection accuracy}\hfill\\
Although machine learning methods address the learnability issue of rule-based systems and improve alert accuracy, they still suffer from a high amount of false positive alerts \cite{Han_et_al_2}. Rule-based systems produce false positive alerts due to rigid rules and their ability to account for complex patterns or new trends that may not have been explicitly specified. Meanwhile, machine learning methods require high-quality training data for modeling, otherwise, the model will be biased and generate false positive alerts \cite{Han_et_al_2}. As a consequence, \cite{Singh_Best} indicated that nearly half of an investigator's time is spent investigating false alerts in many financial orgamizations. However, generating fewer alerts could provide criminals with chances to circumvent the detection and put financial organizations at risk of non-compliance \cite{Han_et_al_2}.

\textbf{Data quality} \hfill\\
\cite{Chen_et_al.} defined data quality as the system ability to ensure data accuracy, correctness, completeness, and relevance. Data quality issues related to customer information might include missing data, dummy values, and null values. Additionally, misspellings, typically stemming from typographical errors or phonetic mistakes, are also encountered \cite{Chen_et_al.}. The pre-processing component addresses these basic issues with data quality \cite{An}.

\textbf{Difficulty in acquiring labeled data}\hfill\\
As part of Suspicious Activity Reporting (see section \ref{SAR}), flagged transactions are forwarded to the authorities for further evaluation \cite{Han_et_al_2}. The final decision on whether a transaction is dependent on the authorities, but not the financial organizations \cite{Han_et_al_2}. Therefore, financial organizations accumulate a high number of suspicious transactions but often receive no feedback from the authorities regarding the accuracy of their decisions \cite{Han_et_al_2}. This means that the data the financial organizations obtain is noisy and often comes without a label of “suspicious” or “legitimate". Without true positive and true negative class, it is difficult to construct models for predicting fraudulent transactions \cite{Han_et_al_2}. To address this issue, \cite{Han_et_al_2} suggested using human analysts' inputs as a feedback loop to improve model training. Because the analysts' input may be the only source accessible for understanding the system's performance, it is critical to consult with them while developing a solution for AML \cite{Han_et_al_2}. 

\textbf{"Human out of the loop" design}\hfill\\
Human investigators play an important role in AML investigation. As mentioned in section \ref{AMLworkflow}, it is a legal requirement for financial organizations to have the final decision on a transaction performed by human agents \cite{Han_et_al_2}. Therefore, many financial organizations still require substantial human resources to address the alerts generated by the detection system \cite{Han_et_al_2}. However, multiple systematic literature reviews have shown that research has tended to focus on optimizing the algorithms to minimize false positive alerts in the field of AML \cite{Chen_et_al.}\cite{Goecks}\cite{Mohammed}. This approach only provides solution for a part of AML investigation workflow and leaves out the \textit{Operational Layer} (see section \ref{AMLworkflow}). Despite the need for human analytical capabilities in the \textit{Operational Layer}, few researchers have focused on providing a human-centered approach for AML \cite{Han_et_al_2}. As a consequent, the reviewing process is still manual and time-consuming \cite{Han_et_al_2}. During this process, the AML investigators must manually perform media search, name screening and researching existing criminal database and sanction lists to find a record match, as well as review the links between multiple accounts \cite{Han_et_al_2}. Spreadsheets are frequently used by analysts to analyze massive data tables \cite{Singh_Best}. Despite offering a thorough perspective of transactions, spreadsheets do not clearly show patterns and relationships \cite{Singh_Best}. Altogether, the manual process causes a significant backlog and frequently an excessive amount of work for the human investigators \cite{Han_et_al_2}.

\textbf{Machine learning interpretability}\hfill\\
Interpretability refers to the model's capability to describe the internals of a system in a way that is understandable to humans. \cite{Gil}. Interpretability is important for AML human investigators because as a part of Suspicious Activity Reporting, the authorities require financial institutions to provide comprehensive and concrete reasoning in their reports \cite{Chen_et_al.}. Therefore, financial institutions need a detailed record-keeping system to provide an audit trail to the authorities \cite{Han_et_al_2}. However, in their systematic literature review, \cite{Kute} found that there is a trade-off between model accuracy and interpretability in AML investigation, in which interpretability decreases as model accuracy rises \cite{Kute}. Unfortunately, ensuring model interpretability has not gotten as much attention in research as enhancing model accuracy \cite{Kute}. Machine learning models' lack of transparency, interpretability, and explainability makes it difficult for them to be adopted, especially in a high-risk industry like finance, whereas the machine learning decision has an important impact on human lives \cite{Kute}. Given that many high-accuracy machine learning models are black boxes, it is difficult for human investigators to build trust in machine learning-enabled systems and include the model results in their Suspicious Activity Reporting \cite{Kute}. 

%evanthiadimara Dimara: I see the connection  but needs to become a bit more explicit from the previous paragraphs,. What re the specific human capabilities (i.e. tasks) that  humans are needed? For example, there is manual rudimentary, debugging algorithm,  high level judgment (e.g. to catch a smart criminal), certain types of search? I guess you one of the high-level tasks should be a decision that involves all (some) of the above? Such claims need to be supported either by citations or by well crafted logical arguments based on citations.

While there are several methods to automate the investigation, interpretability is often omitted from the system design \cite{Kute}. Without interpretability, AML investigators wouldn't be able to provide a rationale that supports their decisions when reporting suspicious activities to the authorities \cite{Kute}. Since AML investigators are legally required to make the final decision on the legitimacy of a transaction \cite{Han_et_al_2}, their decision making process shouldn't be taken lightly. As a result, financial institutions need a new approach to improve machine learning interpretability and take the decision making process of human reviewers into account. 

\subsection{Decision making in AML investigation}
In order to understand why decision making is essential for AML investigation, this section explores decision making theories and examines how it can be applied to the field of AML.

\subsubsection{What constitute a decision task?}\hfill\\ \label{decision task}
Before we delve into the AML topic, we will first examine the basics of decision making and its components.

\cite{Simon} introduced three activities of decision making, including \textit{Intelligence, Design, and Choice}. \textit{Intelligence} refers to the problem identification process, which is carried out by gathering information that may impact the decision. After a decision maker gathers insights about the problem, he/she can evaluate the potential solutions in the \textit{Design} process. The \textit{Design} process is followed by \textit{Choice}, in which the decision maker judge between solutions and select the best solution based on a set of criteria. As a result, the aim of decision making is to investigate, synthesize, and then choose between several potential alternatives. \cite{Dimara_Stasko}

While there are various definitions of decision making, \cite{Dimara_Stasko} defined a \textit{decision making task} as a task in which the human user intends to derive an ultimate choice of direction as a final outcome. They also argued that decision making is a user task that should be aided by visualization, in which the decision could not be supported by automation alone. \cite{Dimara_Stasko}’s argument was an extension of \cite{Simon}’s work, which underlined that decision making should not focus solely on statistics but should also consider human psychology and other environmental variables \cite{Simon}. 

\subsubsection{How is the current decision making process in AML investigation?}\hfill\\ \label{decision}
The next step is to examine the decision making process used in AML investigations and identify its shortcomings. 

\cite{Gao_Xu} developed an AML conceptual model based on Simon's decision making process model. The model consists of five agents: \textit{Data Collection, Money Laundering Monitoring, Behavior Diagnosing, Reporting, and User Agent}. While the first four are automated intelligent agents, only the User agent requires human intelligence. As can be seen in figure \ref{fig:Gao_Xu}, these agents are divided into three groups: Intelligence, Design, and Choice. Data Collection and Money Laundering Monitoring Agents are part of the Intelligence phase, in which the automated system gathers and monitors client and transaction data. If the system detects an unusual client or transaction, the system will forward data to the Design phase. In this phase, the Behavior Diagnosing Agents evaluate risks by identifying existing money laundering patterns and learn to detect new criminal schemes. If there is suspicion about the case, the Reporting Agent will transfer the report to the dedicated personnel with the evidence attached. The human experts only involve in the Choice phase, which they need to make the final decision about the case. Although the human user is also an agent in the decision making process, \cite{Gao_Xu} only discussed the four other intelligence agents and omitted the human user from the system design. 

However, \cite{Han_et_al_2} criticized this workflow and stressed the need for a new workflow that leverages both automation and human decisions. There are several reasons why \cite{Han_et_al_2} are in favor of this argument. Firstly, humans are legally required to remain the ultimate decision makers in AML workflow (see section \ref{AMLworkflow}). Secondly, AML machine learning models suffer from the lack of labeled data, forcing them to rely on the validation of human investigators \cite{Han_et_al_2} (see section \ref{MLchallenges}). Meanwhile, AML investigators still find themselves dedicating significant time to manual information search and aggregation, a process that could be enhanced through automation \cite{Han_et_al_2}. Therefore, a human-computer collaboration might reduce the number of transactions that an investigator must review over time, while improving the performance of machine learning models \cite{Han_et_al_2}.  

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/Gao and Xu.jpg}
    \caption{\cite{Gao_Xu}'s decision making process model for AML}
    \label{fig:Gao_Xu}
\end{figure}

\subsubsection{What are the decision tasks for AML investigators?}\hfill\\ \label{AMLtasks}
As mentioned in section \ref{MLchallenges}, the lack of a human-centered design is a significant problem in the current machine learning systems for AML. Therefore, we will identify the tasks of AML investigators and look into visualization as a potential solution to support AML tasks. 

\cite{Munzner2} suggested that information visualization is necessary when there is a need for augmenting human capabilities instead of replacing them with computational decision making methods. In the case of AML investigation, there are several tasks that human capabilities can be augmented with visualization. For instance, \cite{Singh_Best} mentioned that through effective visualization, AML investigators can gain insights and understanding into large volumes of data \cite{Singh_Best}. The AML investigators' tasks also entail aggregating multiple sources of information \cite{Han_et_al_2}, identifying abnormal patterns \cite{Singh_Best}, and collecting interpretable rationale for reporting \cite{Han_et_al_2} \cite{Kute}. As mentioned in previous section, the ultimate task of AML investigators is to determine if an alert is suspicious \cite{Han_et_al_2}. Therefore, we aim to examine the use of visualization in the AML area as a decision support tool. Further elaboration on the effectiveness of visualization in assisting decision making process will be provided in the next section.

\subsection{Visualization techniques for decision making}
% \evanthia{add an effective subsection outline motivated from the previous section. If not  impossible,  remove/retsructure section}. 

To assess the effectiveness of visualization to support decision making in AML investigation, it is necessary to first understand the role of visualization in the decision making process within an organization. This section presents various visualization techniques that can enhance organizational decision making.

%evanthiadimara Dimara: I am not sure if the introduction i a good objective here. Seems like you plan to give a course on visualization. the point is to introduce the bits of vis research that are relevant to your problem (and of course inevitably define/explain what infovis is, but this is not the main objective, it is means to an end)

\subsubsection{What is information visualization?}\hfill\\
As there are several definition of information visualization, this section emphasizes the specific definition that will be adopted to refer to information visualization throughout this paper.

\cite{Card_1999}, who played a key role in developing the first Graphic User Interface (GUI) that served as the foundation for modern graphic interfaces used in computers today has defined \textit{visualization} as \textit{"The use of computer-supported, interactive, visual representations of abstract data to amplify cognition”} \cite{Card_1999}. Meanwhile, \cite{Singh_Best} defined \textit{Information visualization} as \textit{"the technologies that assist users to “see information in order to help them better understand and contextualize”}. Although being worded differently, both \cite{Singh_Best} and \cite{Card_1999} indicate that visualization can enhance the audiences’ understanding of abstract and complex data. Similarly, \cite{Keim} indicated that information visualization is useful for both showing essential information in large volumes of data and for guiding complex analyses. 

\subsubsection{How can visualization assist decision making?}\hfill\\ \label{visdm}
Information visualization can be used to assist decision making in several ways.

According to \cite{Ware}, information visualization aims to assist the users in:
\begin{enumerate}
    \item comprehending huge amounts of data;
    \item allowing the perception of emergent properties that were not anticipated;
    \item enabling problems with the data to become immediately apparent, such as errors and artifacts in the data;
    \item facilitating understanding of both large-scale and small-scale features of the data;
    \item facilitating hypothesis formation.
\end{enumerate}

It can be seen that the goals of information visualization are closely linked to the three major tasks in decision making (\textit{Intelligence, Design, and Choice}). Dealing with large amounts of complex data can be overwhelming and difficult to comprehend when making decisions. Therefore, a decision maker can use information visualization to \textit{(1) comprehend huge amounts of data} in the Intelligence process. This way, the decision maker can simplify the process and identify the problems quicker. As part of the Design process, the decision maker can assess possible solutions using information visualization to \textit{(2) allow the perception of emergent properties that were not anticipated} and \textit{(3) enable problems with the data to become immediately apparent, such as errors and artifacts in the data}. Since data is presented in a visual form, this decision maker can identify the patterns and anomalies that might not be immediately apparent from raw data. In the Choice phase, the decision maker is presented with multi-attribute choice tasks \cite{Dimara_Stasko}. Information visualization may assist the users to achieve those tasks by \textit{(4) facilitating understanding of both large-scale and small-scale features of the data} and \textit{(5) facilitating hypothesis formation}. Finally, visualization might be applied to reveal how susceptible decision makers are to heuristics and cognitive biases, which can arise when a person faces a choice task \cite{Dimara_Stasko}. 

\subsubsection{What are the visualization needs of organizational decision makers?} \hfill\\ \label{decisionneeds}
Given that the thesis is focused on financial organizations, our research will center on specific needs and preferences regarding visualization of organizational decision makers.

\cite{Baumer} indicated that visualizations are mainly designed to support the analytical tasks of analysts. Especially within the organizational context, the target user of visualization is often the data analysts. Data analysts are are primarily responsible for answering questions with data, and their end products may be used to support decision makers \cite{Dimara2021Unmet}. Meanwhile, decision makers, who are responsible for analyzing and making decisions, often rely on analysts to handle data analysis due to the complexity of the task \cite{Baumer} \cite{Dimara2021Unmet}. Unfortunately, existing studies tend to misunderstand decision makers through the perspective of their subordinates \cite{Dimara2021Unmet}. Since existing literature focuses only on visualization and specific analytic tasks, they often lack consideration for the diverse goals that different audiences may have when interacting with the visualization \cite{Baumer}. Consequently, this emphasis on analysis overlooks the various ways in which people may engage with visualizations. According to \cite{Dimara2021Unmet}, the tasks and processes of decision makers differ greatly from those of data analysts, and therefore their visualization tool also needs to be different. 
\cite{Dimara2021Unmet} characterizes decision makers by their needs for:
\begin{enumerate}
    \item \textit{Need for explanation of analyses}: Decision makers wanted to have the explanation of the analyses to effectively communicate the results with a wider audience within their company.
    \item \textit{Need for information reduction}: Decision makers highlighted the importance of presenting only essential information to enable timely decision making.
    \item \textit{Need for qualitative analysis}: Decision makers emphasized a lack of qualitative nuances in their analytical process since some elements cannot be completely quantified and must be taken into account depending on individual situations and informal input.
\end{enumerate}
 According to \cite{Dimara2021Unmet}, it is important for decision makers to have a \textit{"Flexible Data Interfaces"} because existing visualization tools might not have the essential flexibility for decision makers to interact with the displayed data \cite{Dimara2021Unmet}. \cite{Dimara2021Unmet} listed five approaches to improve the flexibility, including \textit{Social actions}, \textit{Input data actions}, \textit{Mapping and presentation actions}, \textit{Processing} and \textit{Interaction mean} .
\begin{enumerate}
    \item \textit{Social actions}: The capacity to interact with other users was regarded particularly crucial by decision makers, who emphasized the need for coordinated analysis based on a common dataset as a basis for collaboration.
    \item \textit{Input data actions}: Decision makers often do not utilize data in its original form. Instead, decision makers need to revisit the data source and reorganize it as a part of the decision making process.
    \item \textit{Mapping and presentation actions}: Decision makers consistently expressed their needs for flow charts, bullet list, decision tree and action-oriented representations that aren't frequently supported by visualization tools.
    \item \textit{Processing}: In this category, decision makers expressed their needs for guidance when there is substantial data processing involved.
    \item \textit{Interaction mean}: Visualization can also increase the cardinality of interaction means with which a user can perform each action to increase flexibility.
\end{enumerate}

\subsubsection{What visualization should be used for organizational decision makers?} \hfill\\ \label{construtivevis}
Previous section has identified the visualization needs of organizational decision makers. In this section, we will explore the appropriate type of visualization for organizational decision makers.

As mentioned in the previous section, \cite{Dimara2021Unmet} suggested that a visualization need of decision makers is to have \textit{"Flexible Data Interfaces"}. To increase the flexible of the information visualization, \cite{constructive} introduced the use of constructive visualization. They defined \textit{constructive visualization} as the act of \textit{"constructing a visualization by assembling blocks, that have previously been assigned a data unit through a mapping"}. Constructive visualization is a novel approach that empowers individuals non-expert in data visualization to create visual representations that they can use to directly engage with datasets \cite{constructive}. This approach allows novice users to develop flexible visualizations and open up new possibilities for engaging with data \cite{constructive}. Constructive visualization achieves those goals by addressing three key challenges. First, it enables individuals to create their own visualizations, granting them the freedom to express their perspectives. Second, it facilitates the publication and sharing of these visualizations, making them widely available for others to explore and learn from. Finally, it encourages discussion and collaboration around the created visualizations, fostering a deeper understanding and analysis of the data \cite{constructive}. The necessary components for constructing a visualization include a set of basic units or tokens that can be linked to data, a token grammar that defines how the attributes of the tokens convey data, an environment for placing the tokens, and an assembly model that describes the constraints and possibilities for assembling the tokens \cite{constructive}. 

\cite{Dimara2021Unmet} also provided suggestions for future visualization tools to support all decision phases (\textit{Intelligence}, \textit{Design} and \textit{Choice}) through the use of \textit{"Interrogator Tools"} and \textit{"Scenario-Based Simulations"} and \textit{"Trade-off Overviews"}, 

To support decision makers in \textit{Intelligence} phase, \cite{Dimara2021Unmet} identified the need for \textit{"Interrogator Tools"}. These tools serve as a means for decision makers to store, organize, and annotate quantitative and qualitative data \cite{Dimara2021Unmet}. Alternatively, interrogator tools can also be used to conveniently iterative, scan, align and recombine various types of information \cite{Dimara2021Unmet}. In the \textit{Design} phase, the decision makers described their need for a tool to support them in synthesizing various choice possibilities so that they can simulate different scenarios and the outcomes of these scenarios \cite{Dimara2021Unmet}. Lastly, \textit{"Trade-off Overviews"} was the preferred visualization for decision makers in the \textit{Choice} phase. This can be done by using visualization techniques that help the decision maker in ranking the decision criteria and visually combining multiple attributes into aggregated scores \cite{Dimara2021Unmet}. 

%evanthiadimara Dimara: too generic? how is this related to your first section? Remember: first senetnce in a paragraph should be

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/nested-model.png}
%     \caption{\cite{Munzner}'s nested four-level model for visualization design and evaluation}
%     \label{fig:nested-model}
% \end{figure}

% \subsubsection{Who are the users of information visualization?}\hfill\\
% The ambiguity in identifying the targeted user group and the lack of specificity may hinder our understanding of user needs and their challenges. This might lead to over-generalizing research outcomes for unintended users in the original research. Therefore, it is important to understand the users of the visualization and their context of use. 

% Within the field of visualization research, the target users of visualization are often divided into two groups: analysts and decision makers \cite{Baumer} \cite{Dimara2021Unmet}. According to \cite{Dimara2021Unmet}, data analysts are primarily responsible for answering questions with data, and their end products may or may not support decision makers. Decision makers, who are responsible for analyzing and making decisions, often rely on analysts to handle data analysis due to the complexity of the task \cite{Baumer} \cite{Dimara2021Unmet}. However, this results in decision makers being understood only through the perspective of their subordinates.

% \cite{Baumer} addressed this limitation and discussed how visualizations are mainly designed to support the analytical tasks of analysts, which can distract from potential audiences or contexts of use. The paper points out that existing literature focuses only on the visualization and specific analytic tasks, instead of considering the diverse goals that different audiences may have when interacting with the visualization. This emphasis on analysis overlooks the various ways in which people may engage with visualizations. According to \cite{Dimara2021Unmet}, the tasks and processes of decision makers differ greatly from those of data analysts, and therefore their visualization tool also needs to be different. 

% \textcolor{red}{\cite{Munzner} also agrees that the designers of visualization tools should have a clear understanding of their target users. \cite{Munzner} puts forward the nested four-level model for visualization design and evaluation (see figure \ref{fig:interview questions}). This model starts with (1) \textit{domain characterization}, in which the designers must learn about the tasks and data of target users in some particular target domain \cite{Munzner}. While previous work has mostly focused on visualization tools that undertake data analysts as the target user group, there is a lack of literature on visualization tools that customized to the needs of decision makers, especially domain-specific visualization tools. For instance, in the field of AML, visualization tools are often studied through the lens of data analysts \cite{Chen_et_al.} \cite{Kurshan_Shen} \cite{Singh_Best} \cite{Zhou}, but the characteristics of decision makers in this domain are not well understood.} 

% \subsubsection{What are the visualization tasks?}\hfill\\
% The second level of \cite{Munzner}'s nested model is (2) \textit{data and task abstractions}, which aim to map the "what" and "why" into generalized terms. In other words, the domain-specific problems and data are translated into a vocabulary of information visualization. 

% \textbf{Data abstraction}\hfill\\
% Data abstraction answers the question of "what" can be visualized. The visualization designers need to identify the \textit{tasks} that users wish to perform and find the \textit{data types} that will support those tasks. Accordingly, the goal of data abstraction is to transform raw data into the appropriate data type for visualization \cite{Munzner2}. The first data type is items. Items are the individual and discrete entities, such as stock, car, cities. Attributes are also a data type, but they are specific properties that can be measured, observed, or logged, for example salary, price, or temperature \cite{Munzner2}. Attribute types could be categorical, ordinal or quantitative. There are also other data types, such as links, positions and grids. A dataset could consist of multiple data types. There are many ways to depict datasets, such as tables, networks/ trees, fields, clusters/ sets/ lists and geometry. Figure \ref{fig:data-type} illustrates the types of data that can be used. 

% \textbf{Task abstraction}\hfill\\
% Meanwhile, task abstraction aims to answer "why" a visualization tool is being used. In this stage, task descriptions from domain-specific language are transformed into abstract form \cite{BrehmerMunzner} \cite{Munzner2}. Task abstraction often includes a set of actions, namely \textit{analyze} (high-level choices), \textit{search} (find a know/ unknown item), and \textit{query} (find out about characteristics of item). 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/data-type.png}
%     \caption{\cite{Munzner2}'s overview of the types of data that can be used}
%     \label{fig:data-type}
% \end{figure}
% Particularly, \textit{analyze} is the act of using visualization to consume or produce information. A user can consume a dataset in multiple ways, such as by discovering new information, presenting information, or enjoying a casual encounter with visualization \cite{BrehmerMunzner}. Meanwhile, producing information refers to tasks intending to generate new artifacts, such as annotation, recording visualization, and deriving data \cite{Munzner2}.

% The second level of actions is to \textit{search}. A user could search for information in many different ways, such as lookup, browse, locate and explore. Lookup is the act of a user searching for known targets and locations, for example, by looking up a word in the dictionary. Meanwhile, locate occurs when there is a known target, but the location is unknown, such as searching for a node in a network. Browse entails searching for a known location but the target is unknown, such as searching within a particular subtree for leaf nodes having few siblings in tree visualization. Explore takes place when both target and location are unknown, for instance when searching for outliers in a scatterplot \cite{BrehmerMunzner}. 

% The last level of actions is \textit{querying}, which entails three scopes: identify one target, compare some targets, and summarize all targets \cite{Munzner2}. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/abstract tasks.png}
%     \caption{\cite{Munzner2}'s multi-level typology of abstract visualization tasks}
%     \label{fig:abstract}
% \end{figure}

% The aforementioned actions often take place in the context of a \textit{target}, which refers to the aspect of the data that is of interest to the user \cite{Munzner2}. An action-target pair is what usually formulates a user task. Some types of actions could apply to all targets, such as trends, outliers, and features. In some other cases, actions are paired with attributes. If the user only deals with a single attribute, the target of interest might be finding distribution of all values for the attribute, or finding the extreme values of this attribute (such as minimum and maximum values in a range). When there are multiple attributes, the target of interest could be the dependency, correlation, and similarity between these attributes \cite{Munzner2}. In some cases, the targets are specific to the data types. For example, with network data, the user would need to understand the structure of the interconnections between nodes and links. However, with spatial data, the common target of user actions is to understand and compare the geometric shape \cite{Munzner2} (see figure \ref{fig:abstract}).

% \subsubsection{What are the information visualization interactions?}\hfill\\
% \textbf{Encoding/ interaction technique design}\hfill\\
% \cite{DimaraPerin} refers to interaction for visualization as \textit{the interplay between a person and a data interface involving a data-related intent, at least one action from the person, and an interface reaction that is perceived as such}. This concept is closely related to (3) \textit{encoding/ interaction technique}, the third stage of \cite{Munzner}’s nested model. The goal of this stage is to design the visual encoding and interaction, which answers the question of "how" to show the data based on the data type and tasks \cite{Munzner2}. \cite{Munzner2} indicates that a visual encoding and interaction can be constructed through \textit{encoding, manipulation, faceting, and reduction}. Figure \ref{fig:abstract} shows an overview of interaction design choices proposed by \cite{Munzner2}. However, \cite{DimaraPerin} argued that \cite{Munzner2}’s approach is task-driven rather than focusing on user intent, which could make it difficult for users to estimate the flexibility of visualization systems.

% Instead, \cite{DimaraPerin} proposed three groups of interactions: \textit{data interactions}, \textit{perceptualization data interactions} and \textit{non-data interactions}.

% \textit{Data interactions} entail input and processing data actions. Input data actions include editing, updating, modifying, and correcting raw data values, whereas processing data actions apply functions to raw data, such as compile, filter, select a subset and query data. \textit{Perceptualization data interactions} entail mapping data actions or presentation data actions. Lastly, \textit{non-data interactions} entail meta, social, and interface data actions. Meta actions include undoing, redoing, recording activities, logging, and changing history, whereas social actions include communication between multiple users, sharing results, and coordinating the data analysis work of multiple groups. Interface actions involve taking notes, organizing, opening and closing, maximizing, and rearranging the interface. Figure \ref{fig:interaction} provides an overview of the interactions that can be used in visualization tools \cite{DimaraPerin}.
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/interactions.png}
%     \caption{\cite{DimaraPerin}'s interactions for visualization tools}
%     \label{fig:interaction}
% \end{figure}

% \subsubsection{What is algorithm design?}\hfill\\
% The last level of \cite{Munzner} nested model is (4) \textit{algorithm design}. The goal of this level is to develop a computational algorithm to automatically carry out the visual encoding and interaction designs. Algorithm design is different from encoding/ interaction design in the sense that it focuses on solving computational issues, while the latter focuses on addressing human perceptual issues \cite{Munzner2}. Therefore, designers should take into account which aspect they want to focus on when evaluating a visualization. While algorithm design evaluates the design based on system performance and the analysis of computational complexity, visual encoding and interaction design analyze results qualitatively with a more human-centered approach \cite{Munzner2}.

% \evanthia{What is the conclusion /take away of this section? }

\subsection{Using visualization to support decision making in the context of AML}
%evanthiadimara Dimara: what do you mean by conceptualizing visualization? I think the previous section was 'too; conceptual. I would suggest that more concretising  is needed
Previous section discusses how information visualization can be used to support decision making from a theoretical viewpoint. In this section, we will delve into the existing visualization tools that can be employed to aid decision tasks within AML field, along with the challenges associated with these tools. 

% \evanthia{same: section outline? what is the connection with previous sections? }

\subsubsection{What information visualization tools are relevant?}\hfill\\
This section evaluates the available visualization solutions that might support the AML investigators' tasks.
As mentioned in section \ref{AMLtasks}, the decision tasks of human investigators can be summarized as:
\begin{enumerate}
    \item aggregating multiple sources of information \cite{Han_et_al_2};
    \item gaining insights into large volumes of data and identify abnormal patterns \cite{Singh_Best}
    \item providing interpretable rationale for reporting \cite{Kute}
    \item deciding the legitimacy of an alert \cite{Han_et_al_2}
\end{enumerate}

% \textbf{Intelligence phase}\hfill\\
% In this phase, the decision makers aggregates internal and external data sources. There are several existing systems both inside and outside of AML domain that help users to comprehend a large amount of data.

\textbf{Using visualizations for data aggregation} \hfill\\
\textit{TopicPanorama} is a visual text analytics tool that helps users develop a full picture of relevant topics that are discussed in multiple sources \cite{Wang}. It efficiently derives consistent graph matching results among multiple graphs, provides a visualization that allows users to examine the matching results, and allows users to incrementally modify the matching results based on their knowledge and information needs \cite{Wang}. However, the tool is limited in the number of corpora that can be visually compared due to visual clutter and limited screen space \cite{Wang}. Therefore, the authors suggest that future studies should aim to extend interactive modification of matching results to topic mining results and design a suitable visualization for more than three corpora \cite{Wang}.

% \textbf{Design phase}\hfill\\
% As discussed in section \ref{decision task}, visualization in the design phase should allow the users to generate possible solutions and evaluate their feasibility and potential outcomes. In the financial context, many existing visualizations focus on helping users to detect suspicious activities. 

\textbf{Using visualizations to gain insights into large volumes of data and identify abnormal patterns} \hfill\\
In the financial domain, many existing visualizations focus on helping users to detect suspicious activities. 

\textit{Dashboard display to detect suspicious cryptocurrency exchange}\hfill\\
\cite{Zhou} proposed an algorithmic framework to detect suspicious accounts in conjunction with a dashboard that displays the algorithm results. The user interface consists of four coordinated visualization components to support transaction supervisors in their daily work, including: algorithm results, the balance changes of cryptocurrencies held by an account, the transaction patterns contained in transactions launched by the account, and the relevant raw transaction records. The system includes an abacus-inspired visualization to help supervisors find money laundering clues and deduce the trading tactics adopted by launderers. \cite{Zhou} made use of six different views in the user interface, including a suspicious account list view, a BAV view, a feature list view, a wallet balance view, a transaction pattern view, and a transaction record view. 
\begin{figure}
     \centering
     \includegraphics[width=0.45\textwidth]{figures/Zhou.png}
     \caption{\cite{Zhou}'s dashboard to detect suspicious accounts in cryptocurrency exchange}
     \label{fig:zhou}
\end{figure}

%However, this system lacks guidance and annotations to the system that may hinder the system usability. 

\textit{Node-link visualization to detect suspicious activities}\hfill\\
Similar to \cite{Zhou}, \cite{Singh_Best} agreed that AML investigators should use information visualization to find patterns in the transaction data and detect suspicious activities. However, instead of focusing on analyzing the transaction details, \cite{Singh_Best} selected a node-link visualization to represent the movement of funds between bank accounts. 

%Even though the system is useful to understand the relationship between accounts and patterns in data, there was no user evaluation study conducted and this system has not been studied in the user’s context of use. 
\begin{figure}
     \centering
     \includegraphics[width=0.45\textwidth]{figures/TaxThemis.png}
     \caption{\cite{lin_taxthemis}'s TaxThemis User Interface}
     \label{fig:taxthemis}
\end{figure}
\textit{TaxThemis}\hfill\\
TaxThemis is a system designed for tax auditors to detect tax evasion and suspicious transactions \cite{lin_taxthemis}. It offers various visualizations to support the analysis of these transactions (see figure \ref{fig:fraudauditor}). The Control Panel provides a bar chart to show the daily transaction amounts of related parties and allows users to interactively set preferred periods or relevant thresholds to support network fusion. The Group Overview visualizes the topology of related party transactions in each suspicious group and ranks the groups based on their group features, helping users focus on the most suspicious groups. The Graph View displays the hierarchical investment relationships and related party transactions within a selected suspicious group, revealing the common beneficial owners and former tax evaders. Lastly, the Detail View presents the profit status of traders who conducted the selected related party transactions in calendar heatmaps, exposing suspicious behavior such as transferring revenue \cite{lin_taxthemis}. 

\textit{FraudAuditor}\hfill\\
FraudAuditor uses automated algorithms and human experience to perform multi-level fraud analysis, including co-visit network overview, suspicious group identification, and suspicious patient examination. \cite{zhou_fraud} grouped the user analysis tasks into three levels (i.e., overview-level, group-level, and patient-level) (see figure \ref{fig:fraudauditor}). At each level, the authors made use of different visualizations, such as bar charts and node-link diagrams. They selected common and popular charts for several reasons. Firstly, the users are health insurance experts, but they are not familiar with advanced visualizations. In addition, node-link diagrams and graph visualization are used to detect and explore fraud groups because it is an effective visualization to represent interpersonal events. An advantage of this solution is it utilizes commonly used visualization techniques to reduce the amount of time users need to spend learning the system \cite{zhou_fraud}. 

\begin{figure}
     \centering
     \includegraphics[width=0.45\textwidth]{figures/fraudauditor.png}
     \caption{\cite{zhou_fraud}'s FraudAuditor dashboard}
     \label{fig:fraudauditor}
\end{figure}

\textbf{Using visualizations to collect interpretable rationale for reporting} \hfill\\
As mentioned in section \ref{MLchallenges}, interpretability holds significant importance in high-risk sectors like healthcare and finance. Therefore, various studies have focused on machine learning interpretability  within these domains.

\begin{figure}
     \centering
     \includegraphics[width=0.45\textwidth]{figures/RetainVis.png}
     \caption{\cite{Kwon}'s RetainVis visualization}
     \label{fig:retainvis}
\end{figure}
For instance, \textit{RetainVis} is an medical diagnosis software that facilitates interpretability in machine learning models by allowing users to dynamically modify the values of inputs to observe the resulting changes in model predictions \cite{Kwon}. It specifically focuses on providing insights into the contribution scores that make up the risk predictions in medical domain. RetainVis also facilitates user interaction by allowing them to conduct what-if analyses to evaluate and steer the predictive models \cite{Kwon} (see figure \ref{fig:retainvis}). By enabling users to experiment with input changes and observe corresponding output variations, RetainVis enhances the interpretability of the model contribution scores. This interaction also enables users to offer feedback on the contribution scores of individual visits based on their domain expertise \cite{Kwon}. 

%consists of (A) overview of all patients (left) and an attribute summary view (right) of patients; (B) patient summary; (C) patient list, (D) patient editor to conduct a what-if analysis, and (e) patient details

\textbf{Using visualizations to decide the legitimacy of an alert} \hfill\\
\cite{Han_et_al} designed \textit{NextGen AML}, a Natural Language Processing system that makes recommendations for AML analysts by aggregating and analyzing several textual data sources, such as news articles, tweets and criminal records. Aggregated data then got transformed into a time series chart of sentiment trends, graphical distribution of the news articles, and a graph network that represents the relationships between data. By doing so, \cite{Han_et_al} aim to provide additional evidence to human investigators to improve their decision making process. The system provided confidence scores for the analysts to decide whether a transaction was suspicious. 
\begin{figure}
     \centering
     \includegraphics[width=0.45\textwidth]{figures/TUI.jpeg}
     \caption{\cite{TUI}'s Tangible User Interface}
     \label{fig:TUI}
\end{figure}

\textbf{Using constructive visualization to increase flexibility}\hfill\\
Section \ref{construtivevis} discussed the use of constructive visualization to improve the flexibility of information visualization. Drawing inspiration from the research conducted by \cite{constructive}, \cite{TUI} introduced the concept of a \textit{Tangible User Interface}. In this system, users generate queries by positioning and organizing distinct objects on a shared tabletop surface. The visualizations presented on the screen dynamically respond to the arrangement and configuration of the objects on the tabletop. The outcomes of the query are showcased on a monitor positioned at one end of the table (see figure \ref{fig:TUI}). By integrating physical and digital elements, this system creates a highly interactive visualization that facilitates collaboration and empowers users to construct their own data queries.
% \evanthia{As we discussed in the meeting, this should be the main bone of your visualization literature review. The papers that you can build upon,  as well as criticize. You can consider adding the information visualization tools in your section about visualization (perhaps excluding your comments/tools about  decision making. this can be the final conclusion of your visualization review.)\\ I add below  some potential relevant areas for visualization tools (not about decision making, other types of judgment, analysis)  that can be reviewed. But the selection of which ones are more relevant /worth discussion is yours. You can also use your own keywords and find completely different visualization tools.  However, I do expect a considerable number of papers/tools reviewed as part of a MS thesis! The papers I propose below are not only to be cited but to also give you pointers for other papers in their related work. Btw here is an optional course about academic writing in your program, I think Robert took it. You can perhaps consider taking it too if you find it helpful. Some tips can be found here:
% https://sites.umiacs.umd.edu/elm/2019/02/22/writing-the-literature-review/ . Other tips can be borrowed from the  visualization papers which discuss designs and tools. \\\\
% %
% vis  + finance /organizations (but pls find many more than 2) \\ 
% Lin, Yating, et al. "Taxthemis: Interactive mining and exploration of suspicious tax evasion groups." IEEE Transactions on Visualization and Computer Graphics 27.2 (2020): 849-859.\\
% Tovanich, N., Heulot, N., Fekete, J. D., \& Isenberg, P. (2019). Visualization of blockchain data: a systematic review. IEEE transactions on visualization and computer graphics, 27(7), 3135-3152.\\\\
% %
% vis  + fraud detection\\
% Zhou, Jiehui, et al. "FraudAuditor: A information visualization Approach for Collusive Fraud in Health Insurance." IEEE Transactions on Visualization and Computer Graphics (2023).\\\\
% %
% vis + text? (if relevant) \\
% \cite{Baumer} has a reveiw of such papets in their intro (Many of the aforementioned.. .)\\\\
% %
% vis + AI/ML \\
% La Rosa, Biagio, Graziano Blasilli, R. Bourqui, D. Auber, Giuseppe Santucci, Roberto Capobianco, Enrico Bertini, Romain Giot, and Marco Angelini. "State of the Art of information visualization for eXplainable Deep Learning." In Computer Graphics Forum. 2023.\\
% %
% Chatzimparmpas, A., Martins, R. M., Jusufi, I., Kucher, K., Rossi, F., \& Kerren, A. (2020, June). The state of the art in enhancing trust in machine learning models with the use of visualizations. In Computer Graphics Forum (Vol. 39, No. 3, pp. 713-756).\\ 
% %
% Sperrle, F., El‐Assady, M., Guo, G., Borgo, R., Chau, D. H., Endert, A., \& Keim, D. (2021, June). A Survey of Human‐Centered Evaluations in Human‐Centered Machine Learning. In Computer Graphics Forum (Vol. 40, No. 3, pp. 543-568).\\}

\subsubsection{Why do financial organizations need a new information visualization tool?}\label{whyinfovis}\hfill\\
The following section explains the reasons why financial organizations should adopt a new information visualization tool to assist their decision making process in AML investigation.

% While highlighting the importance of user involvement, \cite{Eshet} asserts that users are not just those who use the system, but include all stakeholders whom the system may directly or indirectly impact. As there are many groups of users, identifying all the stakeholders is a prerequisite to user involvement \cite{Eshet}. According to \cite{abras}, a designer must consider a wide range of stakeholders to successfully develop a product. Therefore, a new information visualization tool in the context of AML needs to identify the relevant stakeholders of the decision making process and involve them early in the design and development.

% In addition to user involvement, \cite{Eshet} also highlighted the role of "context of use". \textit{Context of use} refers to the internal and external factors that influence how users interact with a system, such as their goals, motivations, and backgrounds, as well as the resources available to them and the environment they are in. \cite{Eshet} argued that any interactive system would require the users to perform a course of action in order to use the system, and this course of action is always situated within a specific context. Therefore, the usability of a system is dependent on the context of use. Consequently, understanding the user in their "context of use" is essential in order to design interactive systems that are usable, effective, and efficient for users \cite{Eshet}. With that being said, a new AML information visualization tool should not omit the context of use from its design.

\cite{Dimara_Stasko} indicated that the problems with current visualization studies that address decision making are twofold: 

\textbf{Current InfoVis studies often focus on supporting data analysis step rather than decision making}\hfill\\
Firstly, despite decision making is regarded as the ultimate goal of information visualization \cite{Dimara2021Unmet}, visualization task taxonomies very often omit decision tasks by failing to provide assistance on how to study human decisions in the context of data analysis and visualization \cite{Dimara_Stasko}. So far, several studies have been conducted on mitigating decision biases through algorithmic support. However, these studies often focus on supporting data analysis steps rather than decision mechanics, which resulted in a lack of an information visualization tool with a design focus on the decision making process \cite{Dimara2021Unmet}. Accordingly, \cite{Dimara2021Unmet} called for new visualization tools that have more flexibility to support decision flow. 

This finding is also relevant in the AML context. Most studies on AML visualizations \cite{Gao_Xu} \cite{Singh_Best} \cite{Zhou} tended to make no distinction between the decision makers and data analysts. The majority of current AML solutions only focus on supporting analytic activities performed by analysts \cite{Gao_Xu} \cite{Singh_Best} \cite{Zhou}. TopicPanorama \cite{Wang}, NextGenAML \cite{Han_et_al}, TaxThemis \cite{lin_taxthemis} and FraudAuditor \cite{zhou_fraud} all develop their solutions to solve specific analytic tasks such as data aggregation or suspicious activity detection. As established in section \ref{decision}, decision making also plays an important role in the AML process. 
Unfortunately, the existing visualizations lack the flexibility to adequately support the decision making process. For instance, they lack social actions (see section \ref{decisionneeds}) that would enable users to share their work with others. Moreover, the visualizations currently employed for suspicious activity detection lack interpretability, which is essential for AML investigators when reporting to authorities (see \ref{MLchallenges}). Without social actions and intepretability, Suspicious Activity Reporting - an essential part of AML process, is therefore inadequately supported. 

\textbf{InfoVis research lack of evaluation studies whereas the decision makers are the target users}\hfill\\
\cite{Dimara_Stasko} mentioned that the second problem with current visualization is the lack of evaluation studies whereas the decision makers are the target users. As previously mentioned, current AML visualizations often focus on analytical tasks rather than decision making. \cite{Han_et_al} was one of the few authors who focused on developing an AML visualization tool for decision support by using a confidence score. However, the authors have not yet established how the end users make use of the confidence scores in their own decision making process. The authors only briefly described their user evaluation results as “the end users are optimistic” and “their overall feedback and experience have been very positive”. Furthermore, there was no clear indication of whether the target users were data analysts or decision makers. Unfortunately, \cite{Han_et_al} did not provide clear documentation of their user testing regarding decision tasks, leading to the readers’ lack of clear understanding regarding user interaction with the system. In their explanation, \cite{Han_et_al} indicated that due to the sensitivity of the financial businesses, performance metrics were not provided to them. Therefore, future studies on new visualization tools that aim to support decision making process should extend their work and conduct a more in-depth user study.

To address the aforementioned limitations with information visualization, \cite{Dimara_Stasko} suggested that organizations should empower the human decision makers while leveraging the benefits of intelligent technologies. Similarly, within the context of AML, \cite{Han_et_al_2} also advocated for a new workflow that combine human and machine intelligence (see section \ref{decision}). Taken together, when developing a new information visualization tool for AML, here are some directions to explore:
\begin{enumerate}
    \item prioritize the ability to support decision tasks
    \item involve direct input and assessment from decision makers themselves in the evaluation
    \item provide decision makers with the flexibility to construct their visualizations
    \item effectively leverage the capabilities of both humans and machines
\end{enumerate}
The following section describes the methodology used in this study to develop a system that aligns with these objectives.



==> oldUserStudyText.tex <==


\section{METHODOLOGY: DOUBLE DIAMOND DESIGN PROCESS}\label{Methodology}
Building upon the existing related work, this section outlines the methodology employed to design a new visualization tool to support decision making process during an AML investigation. The design has gone through the four phases of the design process, as stated in sections \ref{3-1} (\textit{Discover}), \ref{3-2} (\textit{Define}), \ref{3-3} (\textit{Develop}), and \ref{3-4} (\textit{Deliver}). 

%Figure x depicts the implementation cycles and tools used during each phase of the Double Diamond process.

This study employs the \textit{Double Diamond} design approach, a popular creative process that helps designers and researchers to identify problems of existing technologies and develop innovative solutions \cite{designcouncil}. The Double Diamond approach motivates the designers to question the current state, engage with the problem's context, and gain inspiration from the real experiences of users \cite{kochanowska_double_2022}. What sets this model apart from others is it aligns well with user-centric usability design principles, including the visibility of system status, matching the system with the real world, providing user control and freedom, flexibility, and efficiency of use \cite{doublediamond}. 

The design model consists of four phases: Discover, Define, Develop, and Deliver. As illustrated in figure \ref{fig:doublediamond}, these four phases are represented by two connected diamond shapes. The diamonds represent the problem and solution spaces. Each space goes through a diverging phase that explores different possibilities, followed by a converging phase that narrows down the options \cite{doublediamond}. During the discover phase, the design opportunity are synthesized. In the converging stage that follows, insights and primary design goals are formulated. After generating ideas and creating models in the develop phase, user and expert feedback are collected for evaluation \cite{doublediamond}. The following sections will provide an overview of the methodologies employed in each phase of the Double Diamond design process.

\begin{figure}[ht]
     \centering
     \includegraphics[width=0.45\textwidth]{figures/doublediamond.jpeg}
     \caption{Double Diamond Design Process \cite{designcouncil}}
     \label{fig:doublediamond}
\end{figure}

\subsection{Discover phase: Critical Decision Method}\label{3-1}
This section gives an overview of the Critical Decision Method and its advantages in discovering problems in the current workflow of AML investigators.

The first phase of Double Diamond design process is to discover the underlying problems by talking with relevant stakeholders who are potentially impacted by the problems. The study design makes use of a qualitative approach because it is an effective way to gather requirements and acquire contextual understanding of the current problems \cite{ blandford_qualitative_2016}. Traditionally, interviewing is a popular qualitative method to elicit requirements and domain knowledge from stakeholders. However, there is a lack of prescriptive steps to establish a methodological protocol and re-use the findings beyond the specific study design \cite{cibulski_supporting_2022}. As a result, Critical Decision Method emerged as an extension of current interviewing techniques.

Critical Decision Method encourages the interview participants to reveal their judgments involved in a challenging situation by asking a series of retrospective questions. The technique organizes the interview process into five stages: incident selection, incident recall, timeline construction, and decision point identification. Table \ref{tab:CDM-table} provides an overview of the goals for each stage. 
\begin{table}[ht]
    \centering
    \begin{tabular}{@{}>{\raggedright}p{0.25\linewidth}p{0.7\linewidth}@{}}
        \toprule
        Data Collection Procedure       & Goal \\
        \midrule
        Incident selection & Select a task involving competences beyond routine knowledge \\
        Incident recall & Activate the participants’ memory and to get a first impression of the scenario. The participant is asked to describe the situation from beginning to end \\
        Timeline construction     & The interviewers reconstruct the situation in the form of a timeline \\
        Decision point identification & Identify decision points in the timeline for a detailed investigation \\
        Decision point probing    & Understand the meaning of information for the participant’s assessment of the situation \\
        \bottomrule
    \end{tabular}
    \caption{Five stages of Critical Decision Method}
    \label{tab:CDM-table}
\end{table}
The goal of this study is to discover the cognitive aspects of the current problem-solving strategies that the financial analysts are using to detect financial risks. To achieve this goal, the interview questions are formulated to identify the followings:
\begin{enumerate}
    \item Who is involved in the decision making process?
    \item What are the challenges of the existing financial risk detection applications?
    \item How can visualization involve the financial analysts’ expertise to better solve the current problem?
\end{enumerate}

\subsection{Define phase: User journey mapping and Requirement Analysis}\label{3-2}
This section explores two methods: User Journey Mapping and Requirement Analysis. These two methods are selected to gain a deeper understanding of user experiences and expectations, while also identifying key requirements and criteria for the new visualization tool. 
\subsubsection{User journey mapping}\hfill\\
The focus of the Define phase is on synthesizing the obtained data and extract relevant information to define the design challenges. This phase involves diving into insights, interpreting user emotions and identifying patterns in the user behaviors \cite{kochanowska_double_2022}. A popular method to achieve these tasks is to utilize user journey mapping \cite{moreno_de_oliveira_reporting_2022}. \citet{moreno_de_oliveira_reporting_2022} proposed to harness User Journey in the Define phase to map the user process in each stage of interaction with the tool. The approach starts by breaking down the journey into various phases, each representing a particular event or goal. Once the phases are identified, the user's actions, user's touch points with the system, thoughts, emotions, and potential opportunities for improvement within each phase are reflected in the journey \cite{moreno_de_oliveira_reporting_2022}.

\subsubsection{Requirement Engineering}\hfill\\
While the User Journey Mapping focuses on understanding user interactions, Requirement Engineering goes deeper to identify specific functionalities and features the system needs. It ensures alignment with project objectives, helps prioritize features, and involves stakeholders for a more comprehensive solution. Additionally, it uncovers potential risks and constraints early on, leading to more efficient and effective development. Together, both processes could help the designer to define problems of the current tool and define the scope of the solution.

\citet{Glinz2011AGO} defined requirement engineering as \textit{"a systematic and disciplined approach to the specification and management of requirements"}. To ensure that a software solution correctly solves a given problem, we must first correctly understand and define the problem to solve \cite{lamsweerde_requirements_2009}. Therefore, requirement engineering is established to discover, understand, formulate, analyze and agree on \cite{lamsweerde_requirements_2009}:
\begin{enumerate}
    \item what problem should be solved
    \item why such a problem needs to be solved
    \item who should be involved in the responsibility of solving that problem
\end{enumerate}

\subsection{Develop phase: Creative Problem Solving workshop and Prototyping}\label{3-3}
In the "Develop" phase, we focus on the set up of a Creative Problem Solving workshop and the prototyping process. Through the use of creative problem-solving approaches and iterative development, this phase attempts to explore novel solutions for a new visualization tool.
\subsubsection{Creative Problem Solving workshop}\hfill\\
Brainstorming can be used to bring together stakeholders, users, and designers to collaboratively develop ideas and solutions. According to \citet{treffinger_creative_1995}, Creative Problem Solving (CPS) is a framework that provides individuals or groups with a structured approach to brainstorm. This framework helps participants to address problems and opportunities by formulating the issues at hand, generating and evaluating a wide range of diverse and innovative options, and planning for the successful implementation of new solutions or courses of action \cite{treffinger_creative_1995}. 

CPS process starts with \textit{Understanding The Problem} stage, which the participants attempts to identify and construct the problem statement. Once a problem statement has been formulated, the group would need to come up with a variety of possible options, which \citet{treffinger_creative_1995} referred to this process as \textit{Idea Finding} stage. After the group has identified multiple interesting options, they may require support in refining those options to make an effective choice. Therefore, they can examine the options in \textit{Solution Finding} stage to determine the next steps. In the \textit{Acceptance Finding} stage of CPS, the group would seek out various factors that can either assist or hinder the implementation of potential solutions, such as people, places, materials, and timings that support the plan and contribute to its success. 

\subsubsection{Prototyping}\hfill\\
According to \citet{Silva}, prototyping is an important part of the development process. They highlight several advantages of using prototypes, such as facilitating communication between stakeholders, as well as enabling usability evaluations through inspection and user testing. Prototypes can be derived from user stories and user personas. Throughout the development process, the prototype evolves into a high-fidelity version, which can be used to perform evaluations and usability tests with the end users \cite{Silva}.

If the designer's objective is mainly to use the prototype as a means of communication, only a subset of the overall functionality needs to be implemented. However, when the purpose of the prototype is to conduct user interface testing and validate a specific concept, it should demonstrate a higher level of completeness and fidelity \cite{helander_chapter_1988}. 

The goal of this phase is to gather input on the initial design rather than conducting user testing. Therefore, rapid prototyping is employed to gather feedback quickly. Rapid prototyping is the process of quickly developing tangible representations of ideas to gather feedback and iterate on designs \cite{helander_chapter_1988}. This can be done through low-fidelity prototypes, such as sketches or paper mock-ups, or higher-fidelity prototypes like interactive wireframes or digital mock-ups \cite{helander_chapter_1988}.

\subsection{Deliver phase: Think-aloud usability evaluation}\label{3-4}
The delivery phase employs think-aloud usability evaluation to evaluate the prototype created in the develop phase. The goal of this usability evaluation is to gain valuable insights on the overall user experience and identify areas for improvement to enhance the usability of the new visualization tool.

Usability evaluation involves observing and gathering feedback from users to improve the usability of the software to which they are applied \cite{norgaard}. This technique helps validate design decisions, uncover usability issues, and gather insights for further refinement. The think-aloud is a common protocol for researchers during usability tests \cite{Olmsted}. Think-aloud involves users of an interactive system expressing their thoughts aloud while engaging with the system \citet{blandford_qualitative_2016}. Since think-aloud studies often focus on the interaction with a certain interface, it is an effective way to identify the prototype's strengths and weaknesses as well as how the user perform the tasks using the prototype \cite{blandford_qualitative_2016}. 

\citet{Olmsted} examined and compared various think-aloud protocols: Traditional, Speech Communication, Coaching, and Silent Control. The Traditional protocol involved standard think-aloud with limited probing words and a practice session before testing \cite{Olmsted}. The Speech Communication protocol used verbal feedback like "um-hum" to keep participants talking and probing with feedback tokens or questioning tones after silence \cite{Olmsted}. Coaching protocol included more verbal feedback and direct questions to assist participants, along with a practice session. The Silent Control condition had no think-aloud or probing \cite{Olmsted}. The Coaching protocol resulted in higher success rates and satisfaction ratings, but it introduced bias as participants received assistance \cite{Olmsted}. Therefore, \citet{Olmsted}'s study suggested that practitioners can choose between the Traditional and Speech Communication modes as they did not significantly differ in accuracy or satisfaction ratings. This research opts for the Speech Communication protocol to guide users during tasks because it avoids skewing the task completion rates while maintaining a natural conversational tone.

\newpage
\section{DISCOVER PHASE: CRITICAL DECISION METHOD}\label{section-discover}
In this section, we will discuss the steps taken to discover the visualization needs for AML investigation by conducting a discovery research within a real-world financial organization.
\subsection{Participants}
The initial sample consisted of ten participants. The participants have varying expertise in Anti Money Laundering and financial risk investigation. By doing so, the study could gather insights about the financial risk investigation from different angles. To be eligible for the interview, the participants must:
\begin{enumerate}
    \item have experience in Anti Money Laundering and financial risk investigation;
    \item be comfortable with sharing information about their work routine; 
    \item does not belong to a vulnerable group (physically, mentally, or socially disadvantaged person).
\end{enumerate}
The participants were recruited through a snowball sampling method, in which each participant gave a referral to further participants who might be a relevant stakeholder and satisfy the inclusion criteria. This sampling strategy is selected because it is a quick way to find the participants who have a close approximation to the problem statement \cite{ blandford_qualitative_2016}. Table \ref{tab:interviewee} provides an overview of the interviewees' backgrounds.

\begin{table}[t]
\centering
\begin{tabular}{cccc}
\hline
ID  & Years of experience & Gender & Role \\
\hline
D01 & 1 year 3 months& Male & Transaction monitoring analyst \\
D02 & 3 months & Male & Transaction monitoring analyst \\
D03 & 5 years & Male  & Compliance officer \\
D04 & 3 months & Male & Transaction monitoring analyst \\
D05 & 1 year 4 months & Female & Quality asuarance analyst \\
D06 & 2 year 4 months & Male & Transaction monitoring analyst \\
D07 & 7 months & Female & Transaction monitoring analyst \\
D08 & 1 year & Male & Transaction monitoring analyst \\
D09 & 7 months & Male & Transaction monitoring analyst \\
D010 & 1 year & Female & Transaction monitoring analyst \\
\hline
\end{tabular}
\caption{Overview of the interviewees' backgrounds}
\label{tab:interviewee}
\end{table}
\subsection{Procedure}
The interviews were conducted as follows:

\textit{Part 1: Opening the session}\hfill\\
The opening of this interview aimed to create a welcoming and comfortable atmosphere for the participants. This was achieved by welcoming the participants and thanking them for participating. The interviewer made sure that the participants were feeling comfortable and encouraged participants to ask questions or seek assistance if needed. Then, the interviewer briefly introduced ourselves to build rapport with the participants. 

\textit{Part 2: Introduction to research and getting consent}\hfill\\
In this step, the interviewer provided an overview of the research session to the participants and explained to them what they could expect from this interview. This ensured that the participants understood the research objectives and the activities they would be involved in. Next, the interviewer then explicitly asked the interviewees for consent and informed the participants about the data collection process. 

\textit{Part 3: Main part of Critical Decision Method}\hfill\\
The goal of this session was to discover the cognitive aspects of the current problem-solving strategies that the financial analysts are using to detect financial risks. Several questions were asked during this session in the form of a semi-structured interview. The study followed the critical decision method procedure to create a systematic retrospection of a situation that involved the participant’s expert judgment. \cite{cibulski_supporting_2022}. By going through a past real-world transaction, the participants would reveal the underlying cognitive aspects of their decision making process, such as unobservable knowledge, mental processes, and goals underlying task performance \cite{cibulski_supporting_2022}. Appendix \ref{discovery} lists all the guiding questions being asked in the interviews.

\textit{Part 4: Closing the session}\hfill\\
The interviewer began this part by summarizing the key points and answers that were discussed during the session to ensure that everyone is on the same page. Then, the interviewer encouraged the participants to raise any remaining concerns, suggestions, or additional information they would like to provide. Lastly, the interviewer wrapped up the session and thanked the participants for their time and active engagement throughout the session.

\subsection{Analysis}\label{interview-analysis-section}
There were ten interview sessions overall, each lasting 45 minutes to 1 hour, resulting in ten audio recordings. The audio recordings were first uploaded to the qualitative data analysis platform, \href{https://condens.io/}{Condens.io} to generate transcripts. Then, the transcripts were double-checked manually for higher accuracy. Data management and analysis were also performed using \href{https://condens.io/}{Condens.io}.

The content analysis used the Structural Coding method. Structural Coding is a deductive coding method in which transcripts are classified into a specified set of codes based on interview questions \cite{saldana}. Structural Coding method began with formulating a set of research questions asked during the interviews (refer to appendix \ref{discovery}). Then, these questions were transformed into codes. Based on these interview questions, three primary topics were identified: \textit{the stakeholders involved in the decision making process}, \textit{challenges of the existing tool}, \textit{user needs for the new visualization tool}. In the next step, we thoroughly examined the interview transcripts, extracting relevant data and associating excerpts with the corresponding codes. The fourth step entailed the creation of sub-codes derived from the previously mentioned codes. 

As suggested by \citet{saldana}, other qualitative methods are recommended for further analysis of structurally coded data \cite{saldana}. Therefore, we employed Straussian Grounded Theory as an additional step to conduct an in-depth analysis of the transcripts \cite{corbin}. Straussian Grounded Theory consisted of three stages: Open Coding, Axial Coding, and Selective Coding. During Open Coding, codes were applied to discrete segments of data \cite{corbin}. Subsequently, in the Axial Coding stage, open codes were reviewed and grouped into categories \cite{corbin}. Finally, Selective Coding allowed the us to identify the most significant categories and develop theories based on them. 

After performing qualitative coding, we displayed the finding using the decision requirement table. This table was proposed by \citet{cibulski_supporting_2022} as a representation of the output from CDM method. The decision requirement table specified the "what, how, why, and aid" of the particular decision points. Each column in the table corresponded to a specific decision, while the rows should contain information about why the decision was difficult, how it was made, and what supporting information was used. According to \citet{cibulski_supporting_2022}, the decision requirement table provides insights into the cognitive processes involved in decision making. This information can be used to inform the design of visualizations, interfaces, and interactions that support decision makers effectively.

\subsection{Results} \label{interview-findings}
This section presents the findings from the interviews with AML specialists. These findings were analyzed using the qualitative coding method and are organized in the form of a decision requirement table.

\subsubsection{Qualitative coding}\label{qualitative-coding}\hfill\\
As stated in section \ref{interview-analysis-section}, the findings were categorized into three main categories: \textit{the stakeholders involved in the decision making process}, \textit{challenges of the existing tool}, \textit{user needs for the new visualization tool}. The following section will delve into those categories and present a comprehensive view of the discoveries.

\textbf{Stakeholders}\label{stakeholders}\hfill\\
The decision making process within AML investigation involves three key stakeholders: the AML first-line analysts, the quality assurance analysts, and the second-line compliance officers. Each stakeholder plays a crucial role in ensuring that the organization follows regulatory guidelines and mitigates potential risks associated with transactions made from shoppers to merchants.

The AML analyst is responsible for transaction monitoring and investigating transactions made by shoppers with merchants. Their primary focus is to identify any suspicious activities or patterns that may indicate potential money laundering or illicit financial behavior. The AML analyst utilizes various tools and techniques to analyze transaction data and flag high-risk cases for further investigation. In cases where risks cannot be adequately mitigated at their level, the AML analyst escalates the case to the second line compliance officers.

The quality assurance  analyst ensures the accuracy and efficiency of the investigation process carried out by the AML first line analyst. They review and validate the work performed by the AML first line analyst, ensuring that all processes and procedures are followed correctly. Their responsibilities also include providing feedback to AML analysts to improve their investigation skills and suggesting areas for additional training.

The compliance officer ensures that all AML and regulatory requirements are met. They act as a second line of defense to validate the effectiveness of the AML processes and the work performed by the AML analysts. Compliance officer is responsible for collecting and documenting detailed information related to investigations and reporting, ensuring that all required documentation is maintained. In cases where suspicious activities are confirmed, compliance officers are required to report these activities to the relevant authorities.

\textbf{Challenges of the existing tool}\hfill\\
Throughout the interviews with AML investigators, a range of challenges were identified as follows:

\textit{Lack of documentation}\hfill\\
The interviewees mentioned that the current documentation suffers from fragmentation, disorganization, and a lack of a core system, resulting in inefficiencies and duplicated efforts that hindered the workflow. Valuable information is scattered across various Google documents, leading to knowledge redundancy and missed opportunities for improvement. A compliance officer mentioned:
\begin{quote}
"When we look for information, we need to copy and paste from already existing [project management software]. We do not have a single place where all of this is written down because all the different teams work in different places. We need to scrape the system to look for more context. The system would not document things correctly, they would not group it correctly. So it would be like an exercise of...you just sweep and see what you can find."
\end{quote}

\textit{Difficulty in sense making}\hfill\\
The analysts expressed the difficulty they face in making judgments due to the presence of numerous uncertainties within the AML investigation process. They indicated that decision making involves a substantial amount of human interpretation, which made reaching a decision difficult. Another challenge noted by participants is deciding what to focus on and evaluate, given the huge amount of data available. A compliance officer gave examples when cases were escalated from the first line to the second line due to their difficulties analyzing and comprehending the information provided in the system.
\begin{quote}
"Sometimes first line forwards the case to second line because they cannot interpret what they see in the system"
\end{quote}
As a result, the compliance officer got additional workload and had to spend longer time on the investigation to understand the information provided by the current system. These insights emphasize the significance of building a system that supports AML specialists in efficiently making sense of the information presented to them. 

\textit{Lack of communication}\hfill\\
The interviews also highlighted a problem with communication within the team. Analysts often encountered contradictory information from various teams, leading to confusion and inefficiencies in their decision making process. Additionally, there appeared to be a lack of awareness regarding ongoing projects or initiatives within different teams, resulting in potential overlaps or missed opportunities for collaboration. The communication between the first line and second line analysts was particularly problematic, with participants expressing concerns about its effectiveness. 

\textit{Manual data gathering process}\hfill\\
Throughout the interviews, several significant observations emerged regarding the current automation system's optimization and the challenges faced by analysts. The interviewees expressed that the existing system lacks efficiency, as analysts spend substantial amounts of time searching for information from various sources and manually copying and pasting data. The participants emphasized the need for automation to streamline these manual tasks and enable them to focus on making decisions and identifying patterns. One interviewee expressed that automating the information retrieval process from the internal system to the alert investigation note would be highly beneficial, as it currently involves time-consuming copying and pasting. 
\begin{quote}
"It takes a lot of time for us to copy and paste information from back office to our alert investigation note so automation would be quite helpful"
\end{quote}
Another highlighted the potential for automating the overall account behavior identification process, which currently involves copying and pasting information from various sources:
\begin{quote}
"Most of overall account behavior is just copying and pasting from multiple sources internally and externally. So it would be great to have this process automated. It would also be great to just have the decision to work on, then identify the shopper and the patterns that we see"
\end{quote}
One participant also mentioned the need to reduce the time spent copying existing information from the database and pasting them into their investigation note.
\begin{quote}
Shared information about the merchant's negative media are being stored in Google Docs. We need to manually checking for existing negative media in this database and keep copying information from this Google Docs over.  
\end{quote}

\textit{Lack of flexibility}\hfill\\
The current tool's lack of flexibility presented several significant challenges for the analysts. Firstly, the current tool hindered their ability to tailor it to their specific needs and workflows. The grouping of similar alerts was limited so it only provided a narrow view of the problem, preventing analysts from gaining a comprehensive understanding of the broader context. Consequently, this restricted their ability to make well-informed decisions.

Furthermore, it was observed that the users are dependent on pre-made templates for note-taking. As a result, users typically found themselves needing to incorporate new sentences into the template, which could extend the duration of the investigation process. In some other cases, the templates had redundant information which also take time for the analysts to delete them from their notes. 

Another notable limitation of the current tool was its inefficiency in conducting Open Source Intelligence (OSINT) research. When information is in a different language, analysts faced challenges in gathering and interpreting data, which could significantly impede their investigative process. This language barrier restricted access to crucial information, reducing the tool's effectiveness in handling cross-national alerts.

The current chord diagram and force-directed graph that the users used for AML investigation also suffered from a lack of flexibility, mainly due to its inability to adapt to user preferences and data requirements. Users often encountered issues with irrelevant nodes being connected, making it challenging to derive meaningful insights. Consequently, there is a need for the tool to offer options for removing unnecessary data and conducting quick queries to refine the visualization. The current chord diagram failed to effectively highlight unusual behavior within the network, potentially causing significant findings to go unnoticed. Additionally, the current force-directed graph lacked crucial functionality, as it did not allow users to zoom into nodes and links or interact with them directly, limiting their ability to gain comprehensive insights and hindering effective data analysis. 

\textit{Lack of collaboration}\hfill\\
The absence of a proper collaboration tool posed significant challenges for the team's efficiency and coordination. With scattered tools in use, such as Excel, simultaneous collaboration on the same sheet becomes cumbersome, hindering real-time collaboration. For example, an analyst had already performed an analysis on a shopper, but when there was a new alert concerning the same shopper arose, another analyst must repeat the entire analysis process due to the lack of proper collaboration tool. Consequently, this led to information discrepancies and potential data duplication issues. The lack of a centralized system also resulted in AML investigators unknowingly working on the same alerts or tasks for the same individual, causing duplication of efforts and wastage of resources. 

\textbf{User needs for the new visualization tool}\hfill\\
Throughout the interviews, the interviewees shared several insights on the improvements that they would like to see in the new visualization tool. The following section presents a summary of the user needs expressed during the interviews. 

\textit{Improvement of graph network visualization}\hfill\\
Currently, the AML analysts are using chord diagram and force-directed graph for their analyses. However, the users seek the ability to personalize the graph network according to their specific requirements. The tool should provide a flexible framework that allows users to tailor the graphical representation of data, ensuring a clearer understanding of complex relationships and connections. An user also expressed that the new tool should be enhanced to distinguish between strong links and weak links visually, aiding them in better understanding the relationships and patterns within the data.

\textit{Quick information Access}\hfill\\
Users expressed their needs for a tool that minimizes unnecessary clicks and reduces the need for manual information copying and pasting. By providing quick access to crucial data, they would like the new tool to enables them to perform alert investigations faster. An interviewee particularly requested the ability to click directly on existing transactions to obtain relevant links, eliminating the cumbersome process of querying data from the database as the query takes time and not every analyst has the technical knowledge to do data querying.

\textit{Automation for time saving}\hfill\\
The interviewees indicated that they would like a tool that automates repetitive tasks and accelerates the data aggregation and interpretation processes. By cutting down the time spent on these tedious activities, users can focus more on analysis and decision making.

\textit{Efficient note-taking}\hfill\\
As the AML investigators engage with vast amounts of information, they require a seamless note-taking feature within the tool. By facilitating organized and easily accessible note-taking capabilities, users would be able to effortlessly document their insights and observations during the investigative process.

\textit{Intuitive overview of quantitative data}\hfill\\
User interviews also highlighted the need for a new tool that offers a comprehensive overview of quantitative data, particularly transactional data. Another key aspect that users sought was the ability to determine the frequency of transactions that a shopper make, enabling them to gain a deeper understanding of their transacting behavior. The AML investigators stressed the significance of having the tool process vast amounts of data rapidly while presenting clear and concise visualizations. For example, they would like to have quick access to insights about card usage patterns, transaction velocity, and transaction frequency, presented through user-friendly interfaces. 

\subsubsection{Decision requirement table}\hfill\\
This section presents the decision requirement table that summarized the results derived from the qualitative coding process.

Table \ref{tab:decision-table} provided an overview of the judgements that were involved in performing the observed task using the same approach as \citet{cibulski_supporting_2022}. Section \ref{user-journey} listed out the tasks performed by each user type in their workflow. The interviews showed that there were two decisions required from the users. The first decision is "deciding to escalate the alert," and the second decision focuses on "validating the quality of the decision made by first-line analysts." The decision to escalate the alert could be made by the AML first-line analyst, the quality assurance analyst, and the second-line compliance officer. Meanwhile, the second decision is only made by quality assurance analyst and the second-line compliance officer. 
\begin{table}[t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{2.7cm}p{2.7cm}p{5.8cm}p{4.8cm}}
\toprule
What is the decision? &
Why is it difficult? &
How is it made? &
What is the aid? \\
\midrule
Decide to escalate the alert &
Current tool lacks flexibility &
Analyze the shopper behaviors &
Table displays the transaction list a shopper has made \\
& Available information is difficult to make sense of &
Analyze merchant information &
Chord diagram and force-directed graph display inter-relationships between transactions \\
& Data gathering is manually intensive &
Check negative media on the shopper and merchant &
Search engine \\
& &
Gather data for documentation
&
Internal task management software \\
&
&
&
Shared Google Docs \\
\midrule
Validate the quality of the decision made by first-line analysts &
Lack of tools for collaboration &
Ensure that the analysis is comprehensive and supported by relevant evidence &
Table, chord diagram, force-directed graph, notes \\
& &
Verify that the investigation adheres to regulatory guidelines and internal policies &
Shared Google Docs and Excel\\
& Unclear communication between teams &
Provide feedback to AML analysts to improve and facilitate training &
Internal task management software \\
\bottomrule
\end{tabular}%
}
\caption{Decision requirement table}
\label{tab:decision-table}
\end{table}

In the first decision scenario, which was about escalating an alert, the difficulty arose from several challenges. The current tool lacked flexibility, making it challenging to analyze shopper behaviors and interpret available information. The decision making process also involved analyzing shopper behaviors and merchant information. This task was often aided by a table displayed the transaction list made by a shopper, as well as a chord diagram and force-directed graph to visualize inter-relationships between transactions. The second task involved gathering relevant data, and this process was aided by using internal task management software and shared Google Docs. However, data gathering was manually-intensive, which was time-consuming for the users. As for the last decision task, it entailed checking negative media related to the shoppers and merchants, and for this particular step, the AML specialists often relied on external search engines.

The second decision scenario focused on validating the quality of decisions made by first-line analysts. The compliance officers and AML quality assurance analysts had to make sure the study was thorough and backed up by relevant evidence before making this decision. They would also need to ensure that the analysis followed all internal policies and regulatory guidelines.  However, difficulties might arose from a lack of collaborative tools, which might lead to information discrepancies and potential data duplication issues (for more detail on the challenges, see section \ref{qualitative-coding}). This decision was often aided by the use of a shared Google Docs and Excel spreadsheet. Additionally, the second task involves giving feedback to first-line analysts and supporting their training, which is handled using an internal task management software. A challenge faced in this decision task is the lack of clear communication between teams due to varying user roles, each with its own distinct process. 

\newpage
\section{DEFINE PHASE: USER JOURNEY MAP AND REQUIREMENT ANALYSIS}\label{section-define}
This section describes how we define the design challenges based on the insights obtained during the discovery phase.  

\subsection{User journey mapping}
In the "Define" phase of the Double Diamond design process, the User Journey Mapping is employed to gain deep insights into the user experience of AML investigators and understand their interactions with the current tool.

\subsubsection{Procedure}\hfill\\
To create a user journey map, this study follows the seven-step procedure proposed by \citet{Endmann}. The user journey map is created using the collaborative design tool \href{https://www.figma.com/}{Figma}.

\textit{Step 1: Specifying personas}\hfill\\
Personas represent different types of users who interact with the product or service \citet{Endmann}. Every persona is represented by a digital sticky note containing details about the user, including their job title, years of experience, goal, and pain points. 

\textit{Step 2: Preparing the User Journey Map}\hfill\\
This step involves setting up the visual framework where the journey will be represented. Since there were three user personas, three distinct visual frameworks were created to accommodate each persona's unique journey.

\textit{Step 3: Writing Down the Process’s Associated Activities}\hfill\\
Based on the list of user activities outlined in section \ref{interview-findings}, we arrange these activities in a sequential order to create an outline of the overall workflow for each user persona.

\textit{Step 4: Organizing Activities}\hfill\\
Afterwards, we organize the activities on the user journey map in a logical and cohesive manner to ensure that the activities represent the user's progression through the journey.

\textit{Step 5: Identifying and Naming Tasks}\hfill\\
In this step, the specific tasks that the user performs are identified. These tasks reflect the user's goals and actions during each phase, and they are named concisely and clearly to convey their purpose.

\textit{Step 6: Complementing Activities and Tasks}\hfill\\
The user journey map is then enhanced by incorporating additional information, such as touch points at each stage to offer a more in-depth comprehension of the user's experience. These additional details are derived from the insights obtained during the user interviews.

\textit{Step 7: Assigning pain points}\hfill\\
The pain points obtained from user interviews are then again utilized in this phase to explore and pinpoint the related pain points in each activity for the user. This step helps identify areas where the user journey can be enhanced to deliver a better experience. Based on the number of identified pain points, user emotions were assigned.

\subsubsection{Personas}\label{persona-result}\hfill\\
Based on the interview results presented in section \ref{stakeholders}, there were three user personas defined: AML first line analyst, second line compliance officer and quality assurance analyst. An overview of these user personas can be found in figure \ref{fig:persona}. Figure \ref{fig:journey-1} displayed the user journey of AML first line analysts, whereas figure \ref{fig:journey-2} displayed the user journey of second line compliance officers and figure \ref{fig:journey-3} represented the user journey of quality assurance analysts.
\begin{figure}[ht]
     \centering
     \includegraphics[width=1\columnwidth]{figures/Persona.png}
     \caption{An overview of the user personas}
     \label{fig:persona}
\end{figure}

\subsubsection{Mapping the user journey for each persona}\label{user-journey}\hfill\\
In the workflow of first line analysts, a total of seven activities and fourteen tasks were identified. Figure \ref{fig:journey-1} illustrated that the user journey of AML first line analysts encompassed several pain points, with the highest number observed in the "Shopper investigation" activity. Pain points were particularly evident in areas such as documentation, sense making, data gathering, and data reliability.
\begin{figure}[ht]
     \centering
     \includegraphics[width=1\columnwidth]{figures/journey1.png}
     \caption{An overview of user journey for AML first line analyst}
     \label{fig:journey-1}
\end{figure}

For compliance officers, a total of three activities and twelve tasks were identified. In Figure \ref{fig:journey-2}, the user journey of AML second line compliance officers revealed multiple pain points, with the most prominent ones occurring during the "Investigation" and "Decision" activities. Pain points are notably evident in aspects such as documentation, sense making, data gathering, data reliability and lack of flexibility.
\begin{figure}[ht]
     \centering
     \includegraphics[width=1\columnwidth]{figures/journey2.png}
     \caption{An overview of user journey for AML second line compliance officer}
     \label{fig:journey-2}
\end{figure}

Figure \ref{fig:journey-3} illustrated the workflow of quality assurance analysts. Their workflow comprised four primary tasks and fourteen activities. In comparison to other user personas, they rely more on external tools. Their pain points primarily revolved around challenges with data gathering and the absence of a collaborative tool.
\begin{figure}[ht]
     \centering
     \includegraphics[width=1\columnwidth]{figures/journey3.png}
     \caption{An overview of user journey for AML quality assurance analyst}
     \label{fig:journey-3}
\end{figure}

\subsection{Requirement engineering}
This section presents an overview of the four-step procedure proposed by \citet{lamsweerde_requirements_2009} in requirement engineering, outlining each step's significance and its role in developing an effective software.

\subsubsection{Procedure}\hfill\\
\citet{lamsweerde_requirements_2009} proposed a comprehensive four-step procedure in requirement engineering: \textit{Domain Understanding and Requirement Elicitation}, \textit{Evaluation and Agreement via Negotiation}, \textit{Specification and Documentation}, \textit{Quality assurance}.

\textbf{Domain Understanding and Requirement Elicitation}\hfill\\
This first step of Requirement Engineering focuses on understanding the existing system, including the business organization's structure, dependencies, workflows, and constraints. Within this step, the system designer would evaluate the strengths and weaknesses of the system-as-is. \citet{lamsweerde_requirements_2009} suggested the designer to engage all relevant system stakeholders in the requirements elicitation process to explore the problems and establish improvement objectives. The goal of this step aligns with the discover phase in Double Diamond design process. Therefore, the results obtained from the discover phase can be applied to this particular step (see section \ref{section-discover}).

\textbf{Evaluation and Agreement}\hfill\\
According to \citet{lamsweerde_requirements_2009}, the next step focuses on helping the stakeholders to make informed decisions through trade-off analysis and negotiation, leading to requirements prioritization to determine which features and functionalities are essential for the system. 

A popular approach to represent requirements is using epics and user stories \cite{Lucassen}. \citet{Lucassen} refers to user stories as a method for representing requirements using a simple template such as:
\begin{displayquote}
\textit{“As a [role] , I want [goal], so that [benefit]”}
\end{displayquote}
High-level user stories are grouped by epics to represent features or functionalities of a technical product. Epics serve as containers that capture related user stories, allowing them to be managed and prioritized collectively \cite{lamsweerde_requirements_2009}. In \citet{lamsweerde_requirements_2009}'s findings, user stories have proven to facilitate a shared understanding among stakeholders by encouraging in-depth discussions about requirements. This collaborative approach ensures alignment with end-user expectations within the development team. By accurately identifying the appropriate requirements, the team will be able to develop suitable software. This proactive approach minimizes the need for costly rework, leading to enhanced productivity and improved deliverable quality \cite{Lucassen}. 

Together with a product manager who is responsible for AML technical product development, we compiled a set of epics and user stories for each user persona (see section \ref{persona-result}) based on the findings from the interviews with users. Once the epics and user stories were compiled, the next step was to prioritize them using MoSCoW prioritization method \cite{kravchenko_ranking_2022}. In this method, user stories were corresponding requirement priorities: "must have," "should have," "could have," and "won't have." \cite{kravchenko_ranking_2022}

\begin{table}[t]
    \centering
    \begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}p{2cm} >{\raggedright\arraybackslash}p{8cm} >{\raggedright\arraybackslash}p{4cm}}
        \toprule
        \textbf{Priorities} & \textbf{Description} & \textbf{Matrix axes} \\
        \midrule
        Must have & essential requirements that are absolutely necessary & more frequent and more important \\
        Should have & requirements are important but not critical for the project's success & less frequent and more important \\
        Could have & desirable requirements that would be nice to have but are not vital for the project's success & more frequent and less important \\
        Won't have & requirements that have been deliberately excluded from the project scope due to constraints and project goals & less frequent and less important \\
        \bottomrule
    \end{tabularx}
    \caption{An overview of the categorization for the user stories}
    \label{tab:requirement-priorities}
\end{table}

Afterwards, the user stories would be visualized using a prioritization matrix. The matrix was designed with two distinct axes to aid in decision making and prioritization. The first axis ranged from "less frequent" to "more frequent," categorizing how often a particular user story occurs \cite{Bernardo}. The second axis ranged from "less important" to "more important," signifying the significance of each user story in terms of its impact or value. This matrix allowed the stakeholders to assess the significance and impact of each user story, ranking them based on their importance to the overall project objectives \cite{Bernardo}. Table \ref{tab:requirement-priorities} provides an overview of the categorization for the user stories. 

\textbf{Specification and Documentation}\hfill\\
This phase involves documenting the elicited requirements, providing a clear and comprehensive specification for the system \cite{lamsweerde_requirements_2009}. Based on the user stories elicited from the previous step, we made a documentation that entailed precise definition of all features of the agreed system. By documenting these essential aspects comprehensively, it ensures a clear understanding of the system's scope, functionality, and expected outcome \cite{lamsweerde_requirements_2009}.

\textbf{Quality assurance}\hfill\\
The goal of quality assurance is to ensure the accuracy of the requirements document. Its primary responsibility is to validate the document to make sure it covers all the needs of stakeholders \cite{lamsweerde_requirements_2009}. Thorough checks were performed to find any potential missing parts or inconsistencies, and any detected errors or issues are diligently fixed. By conducting such thorough validation, requirements would be more well-defined and perfectly aligned with the project's objectives \cite{lamsweerde_requirements_2009}.

\subsubsection{Requirement analysis}\label{requirement-analysis-result}\hfill\\
This section presents the requirements gathered through the method outlined in the previous section.

\textbf{Domain Understanding and Requirement Elicitation}\hfill\\
As mentioned in the preceding section, the aim of this step is to evaluate the system-as-is. Based on the qualitative coding results in section \ref{qualitative-coding} and the requirement elicitation, table \ref{tab:requirement-elicitation} provides an overview of the user goals.
\begin{table}
    \centering
    \begin{tabular}{@{}>{\raggedright}p{0.15\linewidth}p{0.8\linewidth}@{}}
        \toprule
        \textbf{Goals} & \textbf{Requirement description} \\
        \midrule
        Goal 1 & Improvement of graph network visualization to better comprehend complex data relationships \\
        Goal 2 & Quick information access to query complex data \\
        Goal 3 & Automation to reduce the time taken to gather data \\
        Goal 4 & Efficient note-taking to reduce time taken to create documentation \\
        Goal 5 & Intuitive overview of quantitative data to get insights for the analysis \\
        \bottomrule
    \end{tabular}
    \caption{An overview of the user goals based on the requirement elicitation}
    \label{tab:requirement-elicitation}
\end{table}

\textbf{Evaluation and Agreement}\hfill\\
In this section, we provide a comprehensive overview of the user stories collected from various user personas. The user stories have been derived from the insights obtained during the interviews with AML specialists and from the discussions with the product manager.

After applying the MoSCoW prioritization method to the epics, we obtained a prioritization matrix that categorized user stories into four distinct groups: Must-haves, Should-haves, Could-haves, and Won't-haves. Figure \ref{fig:Prioritization-matrix} provides an overview of this prioritization matrix. 

Further details of the user stories and prioritization can be found in appendix \ref{define}. Table \ref{tab:US-1} presents an in-depth analysis of the user stories gathered from first-line analysts, providing insights into their specific needs and expectations. Table \ref{tab:US-2} explores the user stories shared by compliance officers and quality controllers, while table \ref{tab:US-3} delves further into the user stories from quality controllers. Finally, in Table \ref{tab:US-4}, we consolidate all of the user stories from across the user personas, providing a comprehensive view of the collective user needs, allowing the designer/ developer to create a solution that meets the different needs of various user personas. 

\begin{figure}[h]
  \centering
  \includesvg[width=0.8\textwidth]{figures/Prioritization matrix.svg}
  \caption{User stories prioritization matrix with four main categories: Must-haves, Should-haves, Could-haves, and Won't-haves}
  \label{fig:Prioritization-matrix}
\end{figure}

\textbf{Specification and Documentation}\hfill\\
This part outlines the specification for quality requirements, also known as non-functional requirements. Quality requirements often include categories such as usability, performance and security. These requirements describe how a system should perform, rather than just what functions it should provide \cite{lamsweerde_requirements_2009}. They ensure that the software not only meets its functional requirements but also delivers a positive user experience and aligns with the broader goals of the project and organization \cite{lamsweerde_requirements_2009}. 

\begin{table}
\begin{tabular}{p{0.5cm}p{13cm}}
\toprule
No. & Usability Requirement \\
\midrule
R1 & The system should create a variety of chart types for interactive visualizations. \\
R2 & The system should implement interactive features like tooltips, zooming, and filtering. \\
R3 & The system should allow visualizations with annotations for insights sharing. \\
R4 & Visual information should be implemented with titles, captions, and contextual information. \\
R5 & The system should ensure responsive design for various screen sizes. \\
R6 & The system should provide users with a range of filter and sorting options that allow them to quickly refine data and arrange results in ways that align with their analytical needs. \\
R7 & The system should export visualizations in Excel and web formats for easy sharing across other users within the platforms. \\
R8 & The system should support collaboration among multiple users on the same project. \\
R9 & The system should provide tutorials, documentation, and user-friendly onboarding. \\
R10 & The visualization should comply with accessibility standards to cater to diverse users. \\
R11 & The system should provide intuitive and efficient navigation mechanisms to allow users to quickly access various sections of the application, including data queries, filters, and visualization settings. \\
R12 & The user interface should be designed to guide users through complex queries without requiring extensive training. \\
\bottomrule
\end{tabular}
\caption{Usability Requirements}
\label{tab:usability-requirements}
\end{table}

\begin{table}
\begin{tabular}{p{0.5cm}p{13cm}}
\toprule
No. & Performance Requirement \\
\midrule
R13 & The interface should respond promptly to user interactions, ensuring minimal delay when applying filters, changing parameters, or executing queries. \\
R14 & The system should optimize memory usage for efficient performance. \\
R15 & Responses to queries shall take less than 1.5 seconds. \\
R16 & The system shall achieve 99.5\% uptime. \\
R17 & The system should be able to handle 10,000 visitors at the same time. \\
R18 & The system should be able to handle 10,000 transactions at the same time. \\
\bottomrule
\end{tabular}
\caption{Performance Requirements}
\label{tab:performance-requirements}
\end{table}

\begin{table}
\begin{tabular}{p{0.5cm}p{13cm}}
\toprule
No. & Security Requirement \\
\midrule
R19 & The system should maintain detailed logs of user activities, actions performed, and system events to track any suspicious or unauthorized activities. \\
R20 & Personal data of the customer shall be collected and stored in compliance with GDPR. \\
R21 & Only AML team members and authorized personnel shall be able to access the alert data. \\
\bottomrule
\end{tabular}
\caption{Security Requirements}
\label{tab:security-requirements}
\end{table}

\textbf{Quality assurance}\hfill\\
Before proceeding with the development of the product, a thorough check was carried out by collaborating with a product manager to ensure that the requirements were of high quality. Any detected errors or inconsistencies were fixed to ensure that the product met the desired specifications and standards. This step was critical in ensuring that the end product would be of high quality and meet the needs of the users.

\newpage
\section{DEVELOP PHASE: CREATIVE PROBLEM SOLVING WORKSHOP AND PROTOTYPING}\label{section-develop}
In the Develop phase, we engage in a CPS workshop and prototyping to foster collaborative solutions.

\subsection{Creative Problem Solving workshop}
After identifying the challenges from the interviews, we facilitated a collaborative workshop involving subject matter experts. This interactive workshop promoted creative thinking and an engaging discussion of ideas, creating a way for effective problem-solving solutions.
\subsubsection{Participants}\hfill\\
The initial sample for the CPS workshop consisted of fourteen participants with diverse expertise in AML. This varied expertise allowed the study to gather insights from different perspectives on AML investigation. The recruitment process for the workshop utilized purposive sampling, which involves selecting participants who are highly likely to provide efficient insights for addressing the research question \cite{blandford_qualitative_2016}. This method was particularly valuable for recruiting participants who had a specific use case and were expected to actively engage with the product of interest \cite{blandford_qualitative_2016}. To minimize individual bias, the process of selecting participants was carried out collaboratively with a product manager who has a deep understanding of the AML team structure. This collaborative approach avoided favoritism or personal biases, which could be a limitation of purposive sampling. By involving the product manager, who has insights into the team dynamics and individual backgrounds, the participant selection process might be more objective and aligned with the overall goals of the study. An overview of the participants who participated in CPS workshop can be found in table \ref{tab:CPS-participants}.

\begin{table}[ht]
\centering
\begin{tabular}{ccccc}
\hline
ID & Experience with AML & Gender & Role & Group \\
\hline
CPS01 & Yes & Male & Transaction monitoring analyst & Group 1\\
CPS02 & No & Male & Product designer& Group 1 \\
CPS03 & No & Male  & Front-end engineer& Group 1 \\
CPS04 & Yes & Female & Back end engineer& Group 2 \\
CPS05 & Yes & Male & Quality assurance analyst r& Group 2 \\
CPS06 & No & Female & Product designer& Group 2 \\
CPS07 & Yes & Male & Transaction monitoring analyst & Group 3 \\
CPS08 & Yes & Male & Product manager & Group 3\\
CPS09 & Yes & Male & Compliance officer & Group 3 \\
CPS10 & No & Male & Product designer & Group 3 \\
CPS11 & Yes & Male & Business analyst & Group 4\\
CPS12 & Yes & Male & Back end engineer & Group 4 \\
CPS13 & Yes & Male & Compliance officer & Group 4 \\
CPS14 & No & Female & Product designer & Group 4\\

\hline
\end{tabular}
\caption{Overview of the participants in the Creative Problem Solving workshop}
\label{tab:CPS-participants}
\end{table}

\subsubsection{Procedure}\hfill\\
CPS workshop was structured as follows:

\textit{Opening the session}\hfill\\
Similar to the interview protocol, it is important to build rapport with the participants during the opening of the session. The session began with the facilitator extended a warm welcome and expresses gratitude to the participants for participating. The interviewer made sure that the participants were feeling comfortable and encouraged participants to ask questions or seek assistance if needed. Then, the facilitator initiated a round of introductions, allowing each participant to briefly introduce themselves and contribute to a sense of familiarity among the group.

\textit{Problem Introduction}\hfill\\
First, the facilitator introduced the user personas, including first line analysts, compliance officers and quality assurance analysts. Then, the facilitator introduced the main problem statement and presents the paint points identified during the interviews. This helped participants grasp the specific challenges that need to be addressed. Afterwards, the facilitator explained the general course of action for the Creative Problem Solving session: (1) idea generation; (2) idea selection; (3) solution finding and (4) acceptance finding. Throughout this process, participants were encouraged to ask questions and seek clarification as needed, ensuring a shared understanding and active engagement.

\textit{Idea Generation}\hfill\\
The goal of this part was to generate a wide range of ideas related to specific problem scenarios. An overview of the problem scenarios being used in this part can be found in appendix \ref{case-guide}. To kick off, participants formed groups based on their roles or areas of expertise, ensuring each group has a mix of different roles. The facilitator then presented the problem scenarios assigned to each group, encouraging participants to generate ideas that address the specific challenges. In guarding the process, the facilitator ensured that everyone had an opportunity to contribute their thoughts and perspectives. As a creative exercise, participants individually drew their ideal investigation tool for the given scenario on paper. This approach encouraged personal expression and exploration of different perspectives within the group. Participants are provided with whiteboards to write down their generated ideas, facilitating simple communication within their groups. 

\textit{Solution Finding}\hfill\\
This stage focused on collaborative discussions and selecting the most promising ideas from the generated list. In a group of four, participants discussed the ideas that they generated individually in the previous stage. Each group reviewed the ideas generated and collectively selects the most promising ones that align with the problem scenario. They then combined their selected ideas to create an interface tailored to each specific scenario. Throughout this process, groups were encouraged to consider the alignment of their ideas with the problem scenario, ensuring that their solutions effectively address the challenges at hand.

\textit{Acceptance finding}\hfill\\
First, participants presented the solutions created by their respective groups. Following that, participants discussed the strengths and weaknesses of each idea.

\textit{Closing the session}\hfill\\
Participants were given the opportunity to ask any final questions or share additional comments they may have. This allowed for any remaining clarifications or thoughts to be addressed before wrapping up the session. Next, the facilitator expressed gratitude once again, acknowledging the participants' active involvement and invaluable contributions of ideas. It was then reiterated that the answers provided during the session would be utilized for qualitative analysis purposes. Lastly, participants were encouraged to reach out to the researchers if they have any further inquiries or wish to provide additional input. 

\subsubsection{CPS analysis}\hfill\\
Since the session made use of digital whiteboards, it generated both textual and visual data. The  analysis aims  to identify and select high-quality ideas that would contribute to the development of a new visualization tool. The following steps were taken to analyze the data:

\textbf{Data collection and merging}\hfill\\
The collected ideas from different sources, including the notes taken during the workshop and digital white boards, were combined into a single list for further analysis. Features and ideas that were mentioned during the sessions but not written on the whiteboards were also collected.
To get a concise list of ideas, duplicate and similar ideas were merged.

\textbf{Questions, Options, Criteria analysis}\hfill\\
Due to the time constraint of the workshop, the evaluation of the workshop results took place separately with the product manager after the workshop, rather than involving the workshop participants directly. However, the product manager's input proved to be very valuable as they had many insights into the feasibility of implementing the potential features. We employed the Questions, Options, Criteria (QOC) analysis method to evaluate the ideas generated from the workshop \cite{qoc}. QOC is a structured framework that helps designers represent design rationale. In the QOC representation, questions are the key design issues that need to be addressed during the design process \cite{qoc}. In this case, questions are defined using the challenges listed in section \ref{qualitative-coding}. Meanwhile, options represent the potential answers or solutions to the questions posed \cite{qoc}, such as the sketches made by the participants in the workshop. An overview of these sketches can be found in figure \ref{fig:workshop-sketch} (appendix \ref{develop}). Lastly, criteria provide a set of evaluation parameters against which the different design alternatives can be measured and evaluated. Three criteria were used in this analysis: \textit{effectiveness in reduce the investigation time for the user}, \textit{benefit to the user} and \textit{ease of use for users}.

\subsubsection{CPS results}\label{CPS-results}\hfill\\
Table \ref{tab:CPS-result-table} displays an overview of Creative Problem Solving workshop results using QOC analysis. The assessment of the "effectiveness in reducing investigation time" relied on the expertise of the product manager, who had a strong background in developing AML solutions. The "benefit" was evaluated based on the five user goals defined in table \ref{tab:requirement-elicitation}. The evaluation of the "ease of use" was grounded in the designer's expertise in human-computer interaction. However, since the users did not evaluate "effectiveness" and "ease of use" criteria directly, further usability evaluation would need to be carried out with the end-users. 

Nonetheless, the CPS workshop provided several insights into the desired features for the prototype. Throughout the workshop, seven key features were consistently proposed by the participants, including \textit{contextual information}, \textit{alert information}, \textit{templates}, \textit{data visualization}, \textit{navigation}, \textit{filter} and \textit{export/ share}. The \textit{contextual information}, \textit{alert information}, and \textit{export/ share} were evaluated as highly effective and easy to use. As a result, the design of the prototype would prioritize these features. 

\begin{table}
\centering
\footnotesize
\begin{tabularx}{\textwidth}{p{1.5cm}p{2.5cm}p{1.5cm}p{6cm}p{1cm}}
\toprule
\textbf{Features} & \textbf{Ideas} & \multicolumn{3}{c}{\textbf{QOC}} \\
\cmidrule(lr){3-5}
 & & \textbf{Effectiveness} & \textbf{Benefit} & \textbf{Ease of use} \\
\midrule
Contextual information & Aggregation of transaction data & High & Automation to reduce the time taken to gather data & Easy \\
 & Shopper summary & High & Intuitive overview of quantitative data to get insights for the analysis & Easy \\
 & Aggregation of shopper behaviors & High & Automation to reduce the time taken to gather data & Easy \\
 & Open source intelligence information & High & Automation to reduce the time taken to gather data & Easy \\
 & Sanction screening information & High & Automation to reduce the time taken to gather data & Easy \\
\midrule
Alert information & Alert category & High & Quick information access to query complex data & Easy \\
 & Alert list & High & Quick information access to query complex data & Easy \\
 & Alert information & High & Quick information access to query complex data & Easy \\
\midrule
Templates & Pre-defined search strings & Medium & Automation to reduce the time taken to gather data & Normal \\
 & Pre-defined workflow template & Medium & Automation to reduce the time taken to gather data & Normal \\
\midrule
Data visualization & Matrix & Medium & Improvement of graph network visualization to better comprehend complex data relationships & Hard \\
 & Bar chart & Medium & Quick information access to query complex data & Easy \\
 & Transaction table & High & Intuitive overview of quantitative data to get insights for the analysis & Normal \\
 & Graph network & High & Improvement of graph network visualization to better comprehend complex data relationships & Easy \\
 & Split view of graph and additional information & High & Quick information access to query complex data & Easy \\
\midrule
Navigation & Segmented control to change view & High & Quick information access to query complex data & Easy \\
 & Tabs & High & Quick information access to query complex data & Easy \\
 & Radial menu & Medium & Efficient note-taking to reduce the time taken to create documentation & Easy \\
\midrule
Filter & Timeline slider & High & Automation to reduce the time taken to gather data & Normal \\
 & Transaction amount filter & High & Automation to reduce the time taken to gather data & Normal \\
 & Make custom query & Medium & Quick information access to query complex data & Hard \\
 & Save custom query & Medium & Quick information access to query complex data & Normal \\
\midrule
Export/ share & Export to Excel & High & Efficient note-taking to reduce the time taken to create documentation & Easy \\
 & Share as a link & High & Efficient note-taking to reduce the time taken to create documentation & Easy \\
 & Write note & High & Efficient note-taking to reduce the time taken to create documentation & Easy \\
 & Save information & High & Efficient note-taking to reduce the time taken to create documentation & Easy \\
\bottomrule
\end{tabularx}
\caption{An overview of Creative Problem Solving workshop results using QOC analysis}
\label{tab:CPS-result-table}
\end{table}

\subsection{Prototyping}
This section describes the prototyping process based on the user stories defined in section \ref{requirement-analysis-result} and the list of desired features in section \ref{CPS-results}.

\subsubsection{Participants}\hfill\\
During the prototyping, the feedback group consisted of one product manager, one front-end developer, one back-end developer, and five product designers. These participants were specifically recruited from the Creative Problem Solving (CPS) workshop. The product manager provided insights into the overall project goals and strategic direction. The front-end and back-end developers brought technical expertise and knowledge of implementation requirements. The product designers contributed their creative skills and user-centered design thinking to address usability issues. Bringing together people with various roles and areas of experience ensured interdisciplinary perspectives for the design. 

\subsubsection{Low fidelity prototype}\hfill\\
The low-fidelity prototype was created based on the sketches and ideas generated during the Creative Problem Solving workshop. The prototype created during this phase included several wireframes. The design tool \href{https://www.figma.com/}{Figma} was being used to create the wireframes. Figure \ref{fig:rapid-prototype} in appendix \ref{develop} provides an overview of the resulting low-fidelity prototype.

\textbf{User flows}\hfill\\
The low-fidelity prototype consisted of automated and manual user flows. The automated flow created a network graph using automation, which allowed users to get a quick and efficient visualization without diving into the details. The manual flow allowed users to have more flexibility in creating their own queries for more comprehensive data analysis. Users could make use of a pop-up modal to select a suitable flow for their needs. Figure \ref{fig:Lofi-popover} illustrates how the users can select the desired investigation flow from the interface. 
\begin{figure}[h]
  \centering
  \includesvg[width=0.7\textwidth]{Low-fi prototype/Lofi-Graph popover.svg}
  \caption{The popover appears as a small window overlaying the main interface that guide users to select between the two options for their desired investigation process}
  \label{fig:Lofi-popover}
\end{figure}

\textbf{Layout}\hfill\\
A split view of the graph and additional information was being used to provide the users with comprehensive overview of the data. By having the relevant information readily available in the same view as the graph, users can save time and effort on navigation (see figure \ref{fig:Lofi-split-view}). 
\begin{figure}[h]
  \centering
  \includesvg[width=0.7\textwidth]{Low-fi prototype/Lofi-Split-view.svg}
  \caption{The split layout interface presents graph on one side and additional information on the other so the users could analyze data simultaneously. (A) The tabs allow users to switch between different sections. (B) The network graph represents the relationships between shoppers and their transaction history. (C) The sidebar displays contextual information that not being shown in the network graph.}
  \label{fig:Lofi-split-view}
\end{figure}

Within the sidebar, the overview tab displayed general information to the users about the graph components, whereas the insight tab provided visualization of transaction data for insight discovery. Figure \ref{fig:Lofi-insight-view} illustrates the data visualization showcased in this tab.
\begin{figure}[h]
  \centering
  \includesvg[height=0.6\textwidth]{Low-fi prototype/Lofi-Insight.svg}
  \caption{The insight tab presents visualization of quantitative data that allows users to analyze data within a single interface}
  \label{fig:Lofi-insight-view}
\end{figure}

\textbf{Features}\hfill\\
Figure \ref{fig:Lofi-manual-view} displays the manual interface that allows users to create and customize queries for in-depth data analysis. Meanwhile, if the users select the automated flow, they will be redirected to the interface shown in figure \ref{fig:Lofi-automated-view}. 
\begin{figure}[h]
  \centering
  \includesvg[width=0.4\textwidth]{Low-fi prototype/Lofi-Manual-view.svg}
  \caption{\textbf{Manual flow:} (A) Shoppers, merchants, and transactions are represented as nodes. Meanwhile, the links represent the relationships between shoppers and merchants (such as purchased from) and between merchants and transaction amount (such as high amount velocity). (B) The time filter allows users to display data within a specified time range. (C) The query filters enable users to extract specific information from the graph by applying custom search criteria}
  \label{fig:Lofi-manual-view}
\end{figure}

\begin{figure}[h]
  \centering
  \includesvg[width=0.4\textwidth]{Low-fi prototype/Lofi-Automated.svg}
  \caption{\textbf{Automated flow:} (A) The side navigation bar helps users to navigate between different pages. (B) The segmented control allows navigation between different views. (C) The tool bar for search, filter, take note, zoom in and zoom out. (D) The checkbox allows users to save information and store it directly into their investigation note}
  \label{fig:Lofi-automated-view}
\end{figure}

\subsubsection{Feedback gathering}\hfill\\
After generating the low-fidelity prototypes, the next step involved collecting feedback from stakeholders, including the product manager of the AML team and developers. By involving these stakeholders, valuable insights and expertise were gathered to evaluate the potential of the prototype. This feedback evaluation played a crucial role in guiding further iterations and refinements of the design, ensuring that the final product would be both practical and aligned with the expectations of the project team. To gather feedback on potential usability issues, the low-fidelity prototype was presented to a group of design experts. The goal of this presentation was to leverage the expertise and critical insights of these professionals in identifying any usability challenges or areas for improvement. Table \ref{tab:feedback-lofi} provides a summary of the feedback gathered from the stakeholders. 

\begin{table}[h]
\centering
\begin{tabular}{>{\raggedright\arraybackslash}p{2cm} >{\raggedright\arraybackslash}p{7.5cm} >{\raggedright\arraybackslash}p{2.5cm}}
\toprule
Category & Feedback & Source \\
\midrule
Feature & Add “share” functionality to make the graph visible to other analysts (such as Excel and link) & Product manager \\
 & Reduce the number of tabs in the segmented control to simplify it & Product manager \\
 & Segmented control should dynamically redirect to different pages based on the type of alert & Product manager \\
 & Add filters for the automated mode & Product manager \\
 & Suggest interesting shoppers based on volume & Product manager \\
User interface & Change the visual encoding of the “save” feature because the checkbox might be confused as a filter & Developer \\
 & Utilize the colors and shape to effectively identify the size of risk & Designer \\
 & Inside the graph, the size of node could correspond to the volume to indicate the transaction volume & Designer \\
 & The components depicted in the graph should align with the content in the right sidebar & Designer \\
 & Add a legend for the visual encoding & Designer \\
\bottomrule
\end{tabular}
\caption{Feedback from the stakeholders on the low fidelity prototype}
\label{tab:feedback-lofi}
\end{table}

\subsubsection{High fidelity prototype}\hfill\\
The development of the high-fidelity prototype was informed by the feedback received on the low-fidelity prototype. This iteration aimed to address the identified usability issues, refine the user interface, enhance the interactive elements, and provide a more polished representation of the AML investigation interface. 

\textbf{User flows}\hfill\\
Based on the feedback from the stakeholders, the manual flow and automated flow were merged into one flow to simplify the user flow. Figure \ref{fig:Lofi-user-flow} shows an overview of this new user flow. In this revised user flow, the user were able to log into their internal software. Afterwards, they could go to a task management page where they could select an open alert to perform investigation. Once they pick up an alert, the user could proceed to alert detail page, where they would document their investigation findings. From the alert detail page, the user could go to graph visualization portal to analyze data with the aid of visualization. 

The interface would then redirect the user flow based on the type of alerts. There were three distinct paths:

\textit{Shopper alert}\hfill\\
Shopper alert refers to the alert triggered by an individual who had unusual purchase behavior. Within this flow, the AML specialists would need to validate why the alert was triggered. Then, the AML specialists could analyze the shopper behaviors with the business from which they made purchases that triggered the alert. The analysts could examine information such as spending patterns or high value transactions, to identify any irregularities that might indicate suspicious activity. The next step in the user flow would be analyzing the shopper behavior at a platform scope, which means the AML specialists would need to analyze the shopper behaviors with all the businesses from which the shopper made purchases before. Lastly, the AML specialists would need to perform Open Source Intelligence (OSINT) search. OSINT describes the act of searching, collecting, analyzing, and using information from open sources like social media platforms, news articles, government publications to gain insights on a particular subject \cite{osint}. The AML specialists could make use of this approach to gain a deeper understanding on the source of fund of a shopper and investigate whether this person was mentioned in any negative media or crime reports. Throughout the investigation, the AML specialists would need to document their whole investigation process to provide evidence for their decision. After they documented the analysis, the AML specialists could do a final examination at the overall behavior of the shopper and make a decision on whether to report this shopper or close the alert.

\textit{Merchant alert}\hfill\\
Merchant alert denotes an alert triggered by a business (such as stores, restaurants, hotels) that has unexplained changes in transaction volume. The analysis process would be similar to the shopper alert investigation, except the focus of investigation would be the business. The AML analysts would need to validate why the alert was triggered on this merchant by examining their business information and transaction history. Afterwards, they would select the shoppers with significant spending patterns to perform further investigation. Then, the rest of the investigation would be carried the same way as shopper alert investigation. 

\textit{Transaction alert}\hfill\\
Transaction alert refers to the alert triggered by abnormal transaction that is inconsistent with the nature of the business or the shopper. In this flow, the AML specialists would need to investigate why an alert was triggered. Subsequently, they would need to analyze the transaction behaviors of the shopper who initiated the flagged transaction. This process involves a thorough examination of their spending history, transaction frequency, and the nature of purchases made. The AML specialists could make use of the manual flow to extract specific information from the graph by applying custom search criteria. Finally, the next steps of the analysis would follow to the same structure as the other flows mentioned earlier.

\begin{figure}[h]
  \centering
  \includesvg[width=1\textwidth]{Low-fi prototype/User flow - V2.svg}
  \caption{An overview of the user flow being used for the high fidelity prototype}
  \label{fig:Lofi-user-flow}
\end{figure}

\textbf{Visual encoding}\hfill\\
In the graph visualization, nodes and edges are employed to represent individual entities and the links between them. Several iterations of the graph were made before arriving at the final design. Along the way, these iterations incorporated various design attributes such as colors, shapes and sizes. Figure \ref{fig:Hifi-graph-iteration} shows an overview of the design iterations for the network graph. 
\begin{figure}[h]
  \centering
  \includegraphics[width=1\textwidth]{Hifi prototype/graph iteration.png}
  \caption{The process of refining the graph visual encoding involved creating multiple versions}
  \label{fig:Hifi-graph-iteration}
\end{figure}

To improve accessibility, the final graph adopted a color palette that mostly consisted of dark grey and red colours. The dark grey color implied low risk, whereas the red color implied high risk. This high contrast color selection aimed to make the graph more accessible and inclusive to a larger audience who might have visual impairments. Furthermore, the red color could signify critical issues that help users quickly identify irregularities within the graph visualization and respond to them. Since there were several information being shown in the graph, the use of colour was kept minimal to reduce the cognitive workload required by the users. Figure \ref{fig:Hifi-graph} presents the final iteration of the graph design.
\begin{figure}[h]
  \centering
  \includegraphics[width=0.6\textwidth]{Hifi prototype/final graph.png}
  \caption{In the final iteration of the graph design, the risk level of each node is displayed through colour variation. Red colour signifies high risk entities, whereas dark grey colour denotes regular entities. The node sizes correspond to the transaction amount: the higher the transactions, the bigger the nodes.}
  \label{fig:Hifi-graph}
\end{figure}

Figure \ref{fig:Hifi-node} presents an overview of the visual encoding being used for the node representation. The network graph included five distinct type of entities: (1) transaction, (2) shopper, (3) sub-merchant, (4) identifier and (5) merchant. The concepts of (1) transaction, (2) shopper and (5) merchant have been introduced previously in this section. Meanwhile, (3) sub-merchant could be business or individual that operates under the umbrella of a primary merchant, allowing them to benefit from the existing payment processing infrastructure of the primary merchant. Meanwhile, (4) identifier refers to the connections that machine learning models establish in order to define a shopper's profile, such as email, IP address and billing address. The visual encoding of the nodes was established in two modes: default and on hover. Default refers to the state in which the users are not interacting with the graph, whereas "on hover" refers to the state that the user's cursor is placed over a node. 

\begin{figure}[h]
  \centering
  \includegraphics[height=0.6\textwidth]{Hifi prototype/Nodes.png}
  \caption{The network graph composed of nodes in five different shapes, each representing a different type of entity.}
  \label{fig:Hifi-node}
\end{figure}

\textbf{Structure of the screens}\hfill\\
Figure \ref{fig:Hifi-information-arch} provides an overview of the information architecture of the interface. The interface's information architecture includes three views: shopper, merchant, and platform. Each view contains four tabs: overview, insight, graph builder, and share. The overview tab aggregates information from multiple sources, allowing users to quickly access information and gain a deeper understanding of why an alert was triggered. The insight tab provides visualization aids such as bar charts, line charts, and tables to analyze transaction data. The graph builder enables the users to manually construct the graph based on their own queries. Finally, the sharing feature allows users to export information as an Excel file or as a link to share with other analysts in the team.
\begin{figure}[h]
  \centering
  \includesvg[width=0.9\textwidth]{Hifi prototype/Information architecture.svg}
  \caption{An overview of the information architecture}
  \label{fig:Hifi-information-arch}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.9\textwidth]{Hifi prototype/Hifi overview tab.png}
  \caption{Screenshot of the overview tab}
  \label{fig:Hifi-graph-overview}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.9\textwidth]{Hifi prototype/Hifi insight tab.png}
  \caption{Screenshot of the graph insight}
  \label{fig:Hifi-graph-insight}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.9\textwidth]{Hifi prototype/Hifi graph builder tab.png}
  \caption{Screenshot of the graph builder}
  \label{fig:Hifi-graph-builder}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[height=0.4\textwidth]{Hifi prototype/Hifi share tab.png}
  \caption{Screenshot of the sharing option}
  \label{fig:Hifi-graph-share}
\end{figure}

When opening the interface, depending on the type of alert, users will be redirected to one of the screens shown in figure \ref{fig:Hifi-graph-overview}. The users can filter the graph based on the transaction amount, transaction method, or identifiers using the filter bar \textbf{(a)}. If the users would like to switch to a different view, they could make use of the segmented control \textbf{(b)}. Within this interface, users can also use tabs \textbf{(c)} to navigate between sections. In the sidebar, users will get a summary encompassing the aggregated information about the alert, shopper, and merchant that is relevant to the alert. Users can make use of the star icon \textbf{(d)} to save relevant information to their notes. Once clicking on the "save changes" button \textbf{(e)}, all changes the users make will be saved to their investigation note and the users will go back to the task management page. The toolbar \textbf{(f)} allows users to search, filter, add annotation to the graph, zoom in and zoom out.

As shown in figure \ref{fig:Hifi-graph-insight}, from the overview tab, the users can switch to the insight tab to facilitate meaningful interpretation with visually intuitive representations, such as charts and tables. Bar chart \textbf{(a)} in the shopper view aims to help the AML specialists make the comparison between pay-ins and payouts of the shopper becomes visually evident. Table \textbf{(b)} provides AML specialists with the means to investigate the transaction history of the scrutinized shopper. In the merchant view, AML specialists can make use of the bar chart \textbf{(c)} to compare the authorized and refused transaction amounts. By using this bar chart, the users would be able to form hypotheses about the past financial activities of the scrutinized merchant. The summary \textbf{(d)} provides users with a baseline of a typical customer profile of this merchant, which would provide more context to the users and help them to gain a better understanding of the merchant business model. In their workflow, AML specialists would need to analyze the shopper behaviors with all the businesses from which the shopper made purchases before. In the platform view, the system would scrape data from multiple sources to provide insights to the AML specialists so that they can quickly access the information they need. The insights include \textbf{(e)} comparison of shopper interaction, \textbf{(f)} total transaction amount, \textbf{(g)} comparison of the transaction amount with all merchants that the shopper has purchased from. 

Figure \ref{fig:Hifi-graph-builder} shows how the users could manually build the graph based on their queries. When they open the graph builder tab, the graph will be in an empty state so that the AML specialists could construct the graph from scratch. They could make use of the \textbf{(a)} "add depth" button to start building the graph. The AML specialists could specify the entity that they would like to see in the graph and define the connections between them using the filters \textbf{(b)} in the sidebar. The users could also make use of the rule builder \textbf{(c)} to create custom queries, such as "show transactions with the high amount and occur more than four times". 

After conducting an investigation, AML specialists can use the share feature shown in figure \ref{fig:Hifi-graph-share}. The users can share findings with team members using a public link or keep it private. They can also download the graph as an Excel document for auditing or reporting purposes.

\newpage
\section{DELIVER PHASE: THINK-ALOUD USABILITY EVALUATION}\label{section-deliver}
In this section, we present an evaluation of the usability test with AML investigators. The goal of this usability evaluation is to gain valuable insights on the overall user experience and identify areas for improvement to enhance the usability of the new visualization tool.

\begin{table}
\centering
\begin{tabularx}{\linewidth}{>{\centering\arraybackslash}p{0.8cm} >{\centering\arraybackslash}p{2.2cm} >{\centering\arraybackslash}p{1cm} >{\centering\arraybackslash}p{3cm} >{\centering\arraybackslash}p{2.5cm}>{\centering\arraybackslash}p{3cm}}
\toprule
ID & Years of experience & Gender & Role & Visualization usage & Graph visualization familiarity  \\
\midrule
UT01 & 8 months & Male & Transaction monitoring analyst & Daily & Intermediate \\
UT02 & 2 years & Male & QA analyst & Daily & Expert \\
UT03 & 6 months & Female  & Transaction monitoring analyst & Daily & Intermediate \\
UT04 & 1 year & Female & Transaction monitoring analyst & Daily & Intermediate \\
UT05 & 1 year & Male & Transaction monitoring analyst & Daily & Intermediate \\
UT06 & 6 years & Male & Compliance officer & Daily & Advanced \\
UT07 & 5 years & Male & Compliance officer & Daily & Beginner \\
UT08 & 9 years & Male & Compliance officer & Rarely or never & Intermediate \\
UT09 & 3 years & Male & QA analyst & Daily & Expert \\
UT10 & 4 months & Female & Transaction monitoring analyst & Daily & Advanced \\
\bottomrule
\end{tabularx}
\caption{Overview of the participants in the usability test}
\label{tab:UT-participants}
\end{table}

\subsection{Participants}
There were 10 participants participated in the usability tests. Each participant had prior experience with AML investigation, with experience ranging from 4 months to 9 years. Similar to CPS workshop, the recruitment process for the usability testing utilized purposive sampling, which involves selecting participants who are highly likely to provide efficient insights for addressing the research question \cite{blandford_qualitative_2016}. The participants were intentionally chosen to represent all three user personas: first line analysts, second line compliance officers, and quality assurance analysts. An overview of the participants can be found in table \ref{tab:UT-participants}. 

\subsection{Procedure}
All usability testing sessions were conducted online via Zoom and were recorded. Following the interaction with the prototype, each participant provided their consent by signing a form and completed the System Usability Scale questionnaire. Then, the facilitator conducted a post-test interview that focused into the participants' experiences with the prototype. At the end each session, the participants were asked to fill out a questionnaire about their background, such as their experiences with AML investigation, as well as their use and familiarity with graph visualization. The usability tests were conducted as follows:

\textit{Part 1: Introduction}\hfill\\
The opening of this session aimed to create a welcoming and comfortable atmosphere for the participants. This was achieved by welcoming the participants and thanking them for participating. Then, the interviewer briefly introduced ourselves to build rapport with the participants. The interviewer made sure that the participants were feeling comfortable and encouraged participants to ask questions or seek assistance if needed. 

\textit{Part 2: Introduction to research and getting consent}\hfill\\
In this step, the facilitator provided an overview of the research session to the participants and explained to them what they could expect from this interview. This ensured that the participants understood the research objectives and the activities they would be involved in. Next, the facilitator then explicitly asked the participants for consent and informed them about the data collection process. An overview of the consent form can be found in figure \ref{fig:consent-form} (appendix \ref{deliver}).

\textit{Part 3: Usability test}\hfill\\
The usability test was divided into two parts: testing the automated graph and testing the manually constructed graph. The first part consisted of ten tasks, whereas the second part consisted of two tasks. An overview of the tasks can be found in figure \ref{fig:usability-test-design}, appendix \ref{deliver}. During the usability test, the participant performed each task step by step, with the facilitator closely observing their interactions. After each part, the participants were asked to fill in the System Usability Scale questionnaire to gauge the overall usability of the prototype. There were ten questions in the questionnaire. Each statement was rated on a scale of 1 to 5, with 1 representing "Strongly Disagree" and 5 representing "Strongly Agree."

\textit{Part 4: Post-test interview}\hfill\\
Participants were prompted to explain their initial interaction with the prototype during the interview session, focusing on what aspects felt positive and what aspects felt challenging or problematic. Participants were then encouraged to describe the possible value and benefits it may provide them in their everyday workflow. To gain a comprehensive understanding of their needs and preferences, participants were asked about any missing functionalities that, if included, would make the portal complete and more useful to them. Lastly, the facilitator asked the participants to provide their ideas on what they would modify in the prototype to better align it with their personal requirements, especially if they were to use it on a regular basis. 

\textit{Part 5: Post-test questionnaire}\hfill\\
In this part, the facilitator requested the participants to complete a short questionnaire about their background and experiences relevant to the study, such as their experiences with AML investigation, as well as their use and familiarity with graph visualization.

\textit{Part 6: Wrap-up}\hfill\\
Participants were given the opportunity to ask any final questions or share additional comments they may have. This allowed for any remaining clarifications or thoughts to be addressed before wrapping up the session. Next, the facilitator expressed gratitude once again, acknowledging the participants' active involvement and invaluable contributions of ideas. It was then reiterated that the answers provided during the session would be utilized for qualitative analysis purposes. Lastly, participants were encouraged to reach out to the researchers if they have any further inquiries or wish to provide additional input. 

\subsection{Analysis}
Ten usability evaluation sessions were conducted, each lasting 1 to 1 hour and 15 minutes. Session recordings were uploaded to the qualitative data analysis platform \href{https://condens.io/}{Condens.io} to generate transcripts. In addition, a questionnaire was sent to the participants before and after the usability tests using \href{https://www.google.com/forms/about/}{Google form}. The results of this questionnaire were documented in an Excel spreadsheet. 

\textit{Step 1: Calculate System Usability Scale (SUS)}\hfill\\
The System Usability Scale (SUS) serves as a valuable tool in assessing usability and customer satisfaction \cite{SUS_aaron}. By providing a single score estimate for overall usability, it enables practitioners to determine the effectiveness of an interface \cite{SUS_aaron}. The scale consists of 10 statements rated on a 5-point agreement scale, which the outcome can range from 0 to 100 \cite{SUS_aaron}. Figure \ref{fig:question-sus} presents an overview of the questions that comprise SUS. 
\begin{figure}[h]
     \centering
     \includegraphics[width=0.6\columnwidth]{Usability test/SUS-ques.png}
     \caption{An overview of questions in SUS}
     \label{fig:question-sus}
\end{figure}
To compute the SUS score, add the contributions from each item, where the contribution ranges from 0 to 4 \cite{Brooke}. For question 1, 3, 5, 7, and 9, the contribution is the scale position minus 1. For question 2, 4, 6, 8, and 10, the contribution is 5 minus the scale position. Finally, we need to multiply the sum by 2.5 to determine the SUS score \cite{Brooke}. The calculation can be represented as the following formula:
\[
SUS \, Score = (Sum \, of \, Odd \, Responses + (5 - Sum \, of \, Even \, Responses)) \times 2.5
\] 

\textit{Step 2: Data encoding using Structural Coding method}\hfill\\
Similar to the interview analysis conducted in section \ref{interview-analysis-section}, the content analysis used the Structural Coding method. As shown in table \ref{tab:excerpt_coding}, we defined five topics using the Structural Coding method: \textit{high severity issues}, \textit{medium severity issues}, \textit{low severity issues}, \textit{positive remarks}, \textit{requests}. We then extracted relevant data from the transcripts and generated sub-codes for each main category. An overview of the sub-codes resulting from this process is available in figure \ref{fig:condens-code}. Each main category has 12 sub-codes labeled 1-12 corresponding to the task numbers.
\begin{table}[h]
    \centering
    \begin{tabular}{p{2cm}p{8cm}p{1cm}p{2cm}}
        \toprule
        Level of Severity & Description & Coding & No. sub-codes \\
        \midrule
        High & User cannot complete task; expresses extreme irritation; needs assistance & H & 12 \\
        Medium & User is frustrated but completes task; suggests potential issues for others & M & 12 \\
        Low & User hesitates or makes a minor mistake; irritation doesn't affect completion & L & 12 \\
        Success & User completes tasks without issues & S & 12 \\
        Request & Feature requests, behavior patterns, interesting user statements & R & 12\\
        Positive & Positive opinions & P & 12 \\
        \bottomrule
    \end{tabular}
    \caption{Excerpt coding categories}
    \label{tab:excerpt_coding}
\end{table}

\textit{Step 3: Analyze data using Straussian Grounded Theory}\hfill\\
The analysis employed Straussian Grounded Theory as an additional step to conduct an in-depth analysis of the transcripts. As explained in section \ref{interview-analysis-section}, Straussian Grounded Theory consisted of three stages: Open Coding, Axial Coding, and Selective Coding. Appendix \ref{deliver} includes figure \ref{fig:tag-group-participant}, which categorizes sub-codes by participant count. 

\subsection{Results}
This section present the results of the usability evaluation with the end-users.

\subsubsection{System Usability Scale}\hfill\\
In this section, we report the SUS score provided by each participant.

The outcomes of the SUS assessments for the ten participants are displayed in figure \ref{fig:overview-sus}. Table \ref{tab:sus_score_ratings} provides a general guideline on how to interpret SUS Score. Part 1 displays results for automated flow, with the system aggregating information for the users. Part 2 displays results for manual flow, where users had to construct the graph using their own queries. Automated flow had an average SUS score of 77, while manual flow had a score of 66.75. According to the SUS scale, a score of 77 indicates good usability. However, a score of  66.75 shows that the system has poor usability and needs improvement. A breakdown of the score for each question can be found in figure \ref{fig:sus-cal}.

Notably, compliance officers with more experience showed a greater interest in the manually constructed graph, while the analysts with less experience favored the automated graph. Noteworthy is the disparity in the manual flow's average score, at 66.75, contrasted with the scores provided by the compliance officers: 82.5, 92.5, and 77.5 respectively. These participants had 5 to 9 years of expertise to the AML field. Conversely, participants with fewer than 3 years of experience exhibited a strong interest toward the automated graph. Only two participants rated the automated flow below average. One had four months of experience and the other had one year of experience and their scores were 62.5 and 57.5, respectively.
\begin{table}[h]
    \centering
    \begin{tabular}{ccc}
        \toprule
        SUS Score & Grade & Adjective Rating \\
        \midrule
        $> 80.3$ & A & Excellent \\
        $68 - 80.3$ & B & Good \\
        $68$ & C & Okay \\
        $51 - 68$ & D & Poor \\
        $< 51$ & F & Awful \\
        \bottomrule
    \end{tabular}
    \caption{General guideline on SUS Score interpretation (\citet{alathas_how_2018})}
    \label{tab:sus_score_ratings}
\end{table}

\begin{figure}[h]
     \centering
     \includegraphics[width=1\columnwidth]{Usability test/SUS calculation.png}
     \caption{An overview of the System Usability Scale questions and answers}
     \label{fig:sus-cal}
\end{figure}

In figure \ref{fig:overview-sus}, daily usage of visualization was reported by the majority of participants, with only one indicating infrequent use. In terms of familiarity with graph visualization, five participants positioned themselves at an intermediate level, while two characterized themselves as experts, another two as advanced users, and one as a beginner. However, this self-reported assessment does not always align with the participants' years of experience or actual usage patterns. For instance, a compliance officer with five years of experience identified as a beginner, while two participants with 2 to 3 years of experience self-identified as experts.
\begin{figure}[h]
     \centering
     \includegraphics[width=1\columnwidth]{Usability test/Overview-participants.png}
     \caption{An overview of the participants and their SUS scores}
     \label{fig:overview-sus}
\end{figure}

\subsubsection{Task analysis}\hfill\\
In the following section, we will discuss the usability challenges faced by users while performing each task during the usability tests.

Figure \ref{fig:ut-tasks} displays the user performance for each task. The majority of users had no significant usability issues in performing task 1,2, 3, 5, and 9. Specifically, task 1 was completed by 7 out of 10 users, task 2 by 8 out of 10, task 3 by 9 out of 10, task 5 by 8 out of 10 and task 9 by 7 out of 10. Only a few participants experienced low to medium usability issues in these five tasks. This result indicates most users can find the graph visualization portal within the internal software, find out why the alert is triggered, identify the most problematic shopper and use the interface to zoom into this particular shopper to facilitate a closer investigation.

For task 6, 7, 8 and 11, the results also indicate varying levels of success among participants. Task 6, which required users to analyze shopper behavior at the merchant scope, shows moderate usability issues. Among the participants, 4 out of 10 managed to complete the task successfully, while one user encountered a low level of difficulty, another faced a medium level, and three users experienced high usability issues. Task 7 asked the users to make use of the filter bar to filter the transactions by emails and billing address. This task had varying outcomes for participants. Among the users, four successfully completed the task, while two encountered low levels of usability issues, two faced medium challenges, and an additional two experienced high usability issues. Task 8 involved evaluating shopper behavior at the platform level. Out of the total of 10 users, four were able to complete the task effectively. However, two users encountered low to medium usability concerns, while another three users faced high usability issues when attempting to undertake this task. Meanwhile, task 11 requested the users to identify the number of alert that the scrutinized shopper had with a particular merchant. The results exhibited a diversified spectrum of outcomes: 3 out of 10 users grappled with high-severity issues, one encountered a medium level of challenge, and five participants succeeded in completing the task proficiently.

The most challenging tasks for the participants were task 4, 10 and 12. Task 4, which required the users to save the relevant information to their investigation, showed that the users were struggling to complete this task. Among the 10 participants, 6 users had high usability issues, 3 of them had medium usability issues and only one user was able to complete this task without guidance from the facilitator. Regarding task 10, which involved decision making, the responses revealed distinct patterns among participants. Notably, 3 out of 10 users expressed a sense of uncertainty, feeling unable to arrive at a decision. Conversely, 6 participants conveyed their need for additional information before making a choice, highlighting the desire for greater clarity. Solely one participant reported having no difficulty in promptly arriving at a decision in this context. Task 12 was also among one of the tasks that posed significant challenges for the participants. The result suggests that 10 out of 12 participants experienced high or medium usability issues with task 12, which required users to manually build graphs with custom queries. In this task, only 2 participants completed the task without issues. 

\begin{figure}[h]
     \centering
     \includegraphics[width=1\columnwidth]{Usability test/Tasks.png}
     \caption{An overview of task performance}
     \label{fig:ut-tasks}
\end{figure}

\subsubsection{Qualitative coding results}\label{results}\hfill\\
As stated in section \ref{interview-analysis-section}, the findings were categorized into five main categories: \textit{high severity issues}, \textit{medium severity issues}, \textit{low severity issues}, \textit{positive remarks}, \textit{requests}. The following section will delve into those categories and present a comprehensive view of the discoveries.

During the usability tests, several observations were recorded. These observations were labeled, grouped, and described in figure \ref{fig:participant-excerpts} (appendix \ref{deliver}).

\textbf{High severity usability issues}\hfill\\
There were four main usability issues that frequently encountered by the users.

\textit{The “save note” feature is often overlookd}\hfill\\
The observation showed that 9 out of 10 users could not find the option to save data points using the star icon without the guidance from the facilitator. Participant 3 indicated the necessity for training or guidance on the functionality of saving data points. Participant 9 concurred with the sentiment, stating that they would also benefit from such guidance:
\begin{quote}
I think I would need the support of a technical person to use the graph...but probably only once. Various functions in this graph visualization were well integrated. The only thing is that the stars that saves your data points would probably need to be more clear. Obviously once it gets shown to you one time, it's fine, you always know that. But it's not immediately obvious because I couldn't even find it. 
\end{quote}
The feedback provided by participants user 3 and user 9 highlighted the need for enhancement within the "save note" feature, which reinforced the importance of enhancing the feature's clarity, ensuring users could easily identify and utilize the functionality.

\textit{The system lacks of interactions that would help users to get more information}\hfill\\
The feedback from participant 3, participant 5 and participant 6 highlighted the need for improved interactions of the visualization. Participant 5 struggled with visual encoding like transaction nodes and identifiers, hindering effective use of the identifier filter. In addition, participant 5 lacked confidence in using the graph because they believe the graph lacked enough information for effective decision making. To address these concerns, this participant suggested to incorporate more labels to clarify node functionality. This user indicated that having labels on nodes upon clicking would increase their confidence in using the graph. 

Participant 6 also agreed that having explanatory labels appear when interacting with nodes would help them understand the nodes better.They  expected to get more comprehensive data, such as historical alerts, KYC records, and transaction details could enhance the usability and value of the graph when interacting with the nodes.

\textit{Graph builder is difficult to use}\hfill\\
The feedback from participant 4, participant 5, and participant 9 highlighted important considerations for refining the usability and accessibility of the graph builder tool. Participant 4 expressed:
\begin{quote}
    This is not quite my way of working. This is for me a little bit going toward the technical side. But I do think that we can all get used to it very easily once we start to understand what we have to do [...] Once I understood, it was easy to use. But I really would need training. And for me, this would require getting used to it because it's more technical. 
\end{quote}
However, when this participant realized that the graph builder had the ability to see all possible interactions with the custom query, the participant was impressed and expressed interest for the graph builder. Participant 4's perspective showed that while the tool initially seemed technical, its potential became evident upon realizing its flexible interaction capabilities. This underlined the need for clearer communication about the tool's functionalities to avoid confusion. 

Participant 5 also emphasized the importance of clarifying the graph's purpose and accessible features from the outset by making users aware of the custom query options. 
\begin{quote}
The graph builder could be useful if you know exactly what you are looking for, but it’s not always the case. I think it will take time to get used to the graph visualization but not necessarily need a technical person to guide it
\end{quote}
Both participant 5's and participant 9's feedback reflected the idea that the graph builder would become useful when used for specific goals, even though it might require some time to get used to. Participant 9 highlighted the significance of accurate labeling for this functionality, alongside a learning curve to fully harness the tool's insights. Participant 9 shared:
\begin{quote}
I did find it a bit hard to use and not because the functionality isn't good. So my feedback here would be...the actual functionality itself is quite good and useful, but just the labeling that you address that functionality is a bit off. I think it has much more actual features that you can extract insights from it. But I think it probably takes more practice to be good at actually getting those insights out of it. It's definitely a change from what you're used to, and I did find the graph builder a little bit challenging to jump into, but I think once you like understand how to use it, it will be fine.
\end{quote}
Overall, these insights stress the necessity of intuitive interfaces, accessible training, and improved communication for seamless adoption of the graph builder.

\textbf{Medium severity usability issues}\hfill\\
Medium usability issues were identified in the user interface's clarity, graph visual encoding, and support for decision making. 

\textit{User interface's clarity}\hfill\\
The placement of icons representing email address and billing address within the sidebar and graph created confusion for user 3, 4 and 6 initially, highlighting the need for more intuitive icon usage. Furthermore, user 4 encountered uncertainty regarding the email and billing address information's placement within the sidebar versus the graph, suggesting a need for clearer cues on where to access relevant information.

\textit{Graph visual encoding}\hfill\\
User 1 struggled with comprehending the visual encoding of transaction nodes. The interpretation of percentage values within nodes posed a challenge for another user, indicating a need for further clarification. The meaning behind graph elements such as entity and level was unclear to user 2, indicating potential issues with terminology and visual indicators. User 3 initially misunderstood the purpose of red icon, associating them with the number of transactions instead of the number of previous alerts. Additionally, user 10 suggested that they had difficulty understanding the significance of the bar graph illustrating model predictions, which could signify a need for improved visualization clarity. 

\textit{External data for decision making}\hfill\\
User 10 indicated that the system lacked support for user-initiated actions like reaching out to merchants for more information, impacting the user's workflow. User 3 expressed the desire to see specific transaction details and sources of funds to facilitate decision making, indicating potential gaps in data presentation. Lastly, user 6 required further external OSINT research to validate the system's conclusions and decisions, which might suggest a need for more comprehensive information from external sources. 

\textbf{Low severity usability issues}\hfill\\
A few instances of low severity usability issues were identified. 

\textit{Navigation}\hfill\\
User 1 was observed spending a long period searching for the graph portal within the internal software, suggesting a potential navigation challenge. Another user encountered confusion surrounding the triggering of alerts, attributing it to an incorrect section they were viewing. 

\textit{Segmented control}\hfill\\
Three user initially grappled with understanding the functionality of the segmented control. However, all of them eventually were able to make sense of this feature and able to use the segmented control for analysis.

\textit{Share analysis as a link}\hfill\\
Another issue arose when users were unsure about the location where their links would be saved. Additionally, two users expressed uncertainty regarding the distinction between public and private links.  

While these issues did not significantly impact the overall usability, they do point to areas where adjustments in user interface design might be beneficial for smoother user interaction.

\textbf{Positive remarks}\hfill\\
The new visualization tool received several positive feedback from all users. 

\textit{The ability to scope down the investigation}\hfill\\
User 6 liked the automated graph's ability to provide an overarching view and assist in scoping activities. 
\begin{quote}
So I think a functionality like this is very nice to get an overview of what is going on. So you could immediately see that, for example, next to the the initial alert for the parking merchant, there are some other things you might need to consider. So it would be very nice to immediately see that and include in your analysis. That will be just more efficient. So yeah, I would definitely make use of it to determine the scope of what you're looking at. I think it provides a very good tool for scoping and then also the way you can click through would make things also a lot of faster. 
\end{quote}

\textit{The easy navigation between different views using a segmented control}\hfill\\
User 3 initially concerned about the tool's impact on the current critical functionalities. Upon realizing the actual capabilities of the new tool, user 3 had a very positive reception. The segmented control feature was well-received by users, although some initial guidance on its usage could further enhance the experience. User 4 liked the segmented control because it helped them easily navigate between the platform view and the shopper view. User 4 indicated that:
\begin{quote}
I think that I would like to use the graphic visualization frequently. Currently, we have a division of a platform, merchant and shopper. I really don't like that...So I would really love that I can just switch this easily. That would really make my life much easier and I think other analysts would agree with that. So I really like the visualization. I would probably need a little bit more explanation on certain things, but I guess that would come at a later stage.
\end{quote}

\textit{The explanation for factors that impacted the model prediction}\hfill\\
A participant was particularly impressed by the feature that provided explanation for the factors influencing the model's predictions. User 9 expressed:
\begin{quote}
Actually very interesting, so I'll go through what I actually really liked. So I really like this, the platform thing, I think this is really useful. What I also liked it showed what factors impact the model prediction. And I think it's also something that people struggle with a bit, so having that there already is like very useful. I like the fact we've got dropdown for all the personal identifiable information. Yeah, I really like the option to share because usually you've got a whole bunch of things selected and if you send to someone they have to do the whole process again. So if you can save a view and send this, I think that's really useful. I actually have quite a positive impression.
\end{quote}
Overall, these positive comments underscore the tool's potential to deliver valuable insights and usability enhancements to users.

\textbf{Requests}.\hfill\\
The requests made by the user can be organized and classified into the following groups:

\textit{Need for efficient note-taking and documentation}\hfill\\
4 out of 10 users gave feedback specifically on the need for efficient note-taking and documentation. They needed efficient methods to document their analysis procedures, categorize information thematically, and save filters for future use. They also desired a system that automatically saves information based on predefined templates and enables them to present notes in a coherent and accessible manner to others.

\textit{Need for transaction list}\hfill\\
Many participants voiced the necessity for a list of transactions to accompany the graph. They emphasized that while the graph provides a visual representation of transaction data, a corresponding transaction list would offer a detailed breakdown of individual transactions and their corresponding amounts. This additional component was seen as crucial for enhancing transparency and facilitating a comprehensive understanding of the transaction information being presented. By incorporating both the graphical representation and the transaction list, participants believed that users would be better equipped to analyze, interpret, and make informed decisions based on the data provided.

\textit{Need for quick access to external data (google search query)}\hfill\\
The necessity for swift access to external data, such as through Google search queries was mentioned by six users. For example, participant 3 indicated that they were inclined to conduct manual searches using open source intelligence to identify negative media, addresses and personal information of the subject under investigation. Additionally, participant 3 was looking for a feature that would enable the validation of shopper and merchant details using external sources, potentially verifying factors like the source of wealth. Additionally, user 8 specifically expressed the importance of direct links to Google Maps for billing addresses. User 10 was interested in a more flexible date filter capturing a emphasized their intent to leverage historical data effectively. 

\textit{Need for advanced filter}\hfill\\
3 out of 10 users expressed the need for advanced filter functionality, such as excluding irrelevant data points and using filter based on geographic location.

\textit{Need for using payment method to identify shopper behavior}\hfill\\
Three users wanted improved shopper behavior analysis using payment method. User 6, 8 and 10 suggested that they needed get essential transaction details to assess transaction behaviors and patterns in the shopper behaviors. 

\textit{Need for more interactions that would provide additional information}\hfill\\
Five users expressed a strong need for more comprehensive information and a richer analytical experience within the system. For example, user 6 requested access to detailed merchant node information, including alert specifics, detection methods, transaction volumes, card details, and transaction particulars. Additionally, user 1, 2 and 4 expressed their wish to zoom in on specific transaction data within the graph and to explore total settled volumes of groups of merchants. The would like to have enhanced interactions like popovers, hover effects, and dynamic opacity highlights the need for dynamic visualization. Lastly, user 7 would like to have the ability to select a group of entity and get an aggregation of the transaction volume based on their selection.

\textit{Need for training and contextual guidance}\hfill\\
7 out of 10 users highlighted a clear need for improved explanation and contextual guidance within the system. Two users indicated that some features, such as the graph builder, was too technical and requested more guidance.  Additionally, users suggested incorporating more labeling and providing clear explanations within the graph builder, recognizing the value of visual aids in enhancing user understanding. The users' requests for guidance in utilizing the graph builder underscore the importance of providing guidance for complex features. Furthermore, users' struggles with visual encoding and filter comprehension in the graph highlight the necessity for intuitive design and informative cues. 

The feedback from participant 4, 5, 6, and 10 also emphasized the importance of implementing comprehensive training and guidance for AML specialists before interacting with the system. The consensus among users underscored the need for guidance on understanding the visual encoding and navigation within the platform. Participant 10 indicated:
\begin{quote}
It's the kind of thing that after a few times of using it, it will become like second nature. For now, being introduced to it. It did feel quite complex, but most of it was useful [...] I think that I would need the support for the 1st 2 uses maybe. After that, maybe for a first alert, if I had someone go through an entire alert doing this graph visualization and then I had like 2 hours to do my first alert with it with like clicking on everything I possibly can to figure it out, then I think I would not need the support of a technical person.
\end{quote}
UT10's feedback highlighted that a learning curve that could transform into familiarity over time. However, they would still need  initial guidance to facilitate a smooth introduction. 

\newpage
\section{DISCUSSION}\label{section-discussion}
%This section interprets the results in the context of the research objectives and related literature. It provides an analysis of the findings, discusses their implications, and explores potential explanations or hypotheses. 
In the discussion, we interpret our findings on the effectiveness of data visualizations in supporting decision making in the context of AML investigation, compare them with existing literature, and explore potential design implications based on the findings.

\subsection{The needs of AML decision makers}
This section explores the unique needs of AML decision makers and compares them to decision makers' needs found in existing literature.

As mentioned in section \ref{decisionneeds}, \citet{Dimara2021Unmet} characterized the organizational decision makers by their needs for \textit{explanation of analyses}, \textit{information reduction} and \textit{qualitative analysis}. Upon evaluating these aspects with AML users, it becomes apparent that they exhibit a need for \textit{qualitative analysis} and \textit{explanation of analyses}, which aligns with the \citet{Dimara2021Unmet}'s earlier findings. However, the result suggests that there is less user needs for information reduction. Moreover, the research broadens the understanding of AML user needs by introducing an additional dimensions: the \textit{need for placing data within broader contexts}. The following paragraphs will discuss these user needs more in-depth.

\subsubsection{Need for explanation of analyses}\hfill\\
Throughout the interviews and usability testing sessions, the AML investigators emphasize the need to communicate their findings to a wider audience. As mentioned in section \ref{SAR}, reporting unusual and suspicious activities is essential for financial institutions to comply with regulatory requirements. Since there are multiple factors that need to be considered when reporting suspicious activity, the authorities require reporting procedure to have clear audit trails that document the actions and decisions being undertaken by the financial organizations. The research reaffirmed this need, as AML investigators repeatedly emphasized the necessity of recording each step and providing comprehensive justifications underlying their decisions. It is clear that AML investigators rely on accurate and efficient reporting procedures. Previously, AML investigators had to manually copying and pasting information from diverse sources into their notes. The proposed new visualization system introduces an efficient way for decision makers, allowing them to promptly record the notes, thereby enabling the direct aggregation of information into their investigative records. 

In accordance with our earlier assumption concerning the limitations of the AML system as highlighted in section \ref{MLchallenges}, the study uncovered machine learning interpretability as a prominent challenge. A user expressed interest in understanding the factors that impacted model predictions and pointed out that other analysts were facing similar struggles. As the validation of why an alert was triggered stands as a mandatory step in the AML investigation workflow, gaining insights into the algorithmic decision by which the model generates alerts holds significant importance. However, the usability testing revealed that not all users were familiar with the concept of machine learning interpretability. Despite the design incorporating bar charts to represent the factors contributing to model predictions, less tech-savvy users encountered difficulties in comprehending this visualization method. To bridge this gap, there's a need for intuitive visual representations that cater to users with varying levels of technical expertise. 

\subsubsection{Need for qualitative analysis}\hfill\\
This section delves into the first organizational decision maker needs mentioned by \citet{Dimara2021Unmet}: the \textit{need for qualitative analysis}.

According to \citet{Dimara2021Unmet}, the decision maker's need for qualitative analysis becomes apparent due to certain aspects that cannot be fully quantified and must be considered based on individual situations and informal input. As outlined in section \ref{results}, users expressed the demand for quick access to external data sources such as Google search queries, public databases, or social media platforms. In the context of AML investigators, despite the system providing a wide range of quantitative data, users still need to conduct OSINT research to make sense of the data. For example, a AML investigator may observe a high frequency shopper, but to gain a comprehensive understanding of their behavior, the decision maker would require additional contextual insights. As a result, the AML investigators often turn to external data resources, including social media presence, addresses, and company profiles, to verify the sources of funds associated with a shopper. This highlights how the quantitative data provided by the system necessitates qualitative exploration for comprehensive decision making.

The need for qualitative analysis was also reflected through the users' requests for training and contextual guidance in section \ref{results}. The result found that users possessed varying degrees of familiarity with the visual encoding employed in the visualizations. While certain users exhibit proficiency, others encounter technical challenges when attempting to utilize advanced features, often deeming them overly technical. Particularly among less technically savvy users, there was a strong preference for a qualitative explanation that would offer greater intuitiveness. This underscores the significance of accommodating diverse user backgrounds and competencies by providing accessible explanations that facilitate a deeper understanding of the visual representations, ultimately enhancing the effectiveness of the decision support system.

\subsubsection{Need for placing data within broader contexts}\hfill\\
The research further introduced another dimension of decision makers' needs: the \textit{need for placing data within broader contexts}. 

Interestingly, the need for placing data within broader contexts closely intersects with the needs for qualitative analysis. For instance, when AML investigators conducted research using external resources, they weren't only looking for qualitative explanation, but also to understand the shopper behaviors in the larger context. As organizations make decisions based on several factors, understanding the larger contexts within which data exists becomes extremely important. This is particularly evident in our findings. Unlike traditional organizational decision makers who often prioritize information reduction to facilitate efficient decision making, AML investigators demonstrated a distinct pattern of needs.

\citet{Dimara2021Unmet} indicated that organization decision makers often emphasized the significance of presenting only essential information to facilitate decision making. However, AML investigators, due to the unique nature of their tasks, exhibited a contrasting requirement. In contrast to the need for information reduction, AML investigators indicated a preference for data with a deeper granularity. The context behind certain behaviors and transactions played an essential role in their decision making process. This compelled them to seek a comprehensive understanding of the data, implying that they preferred gathering as much information as possible before arriving at a decision. While AML investigators were keen on having a comprehensive overview of all the aggregated information accessible in the prototype, they also expressed a desire for more detailed data to be more confident in their decision making process. This could be attributed to the fact that their work is situated within a high-risk domain, where being more assured in their choices is vital. 

As we have a more our refined understanding of decision maker requirements, it is important to have tailored approaches in design and presentation of data to cater to these unique needs. The following section will provide design implications based on the user needs discussed in this section.

\subsection{Design implications for AML investigation tool}
This section conducts a comparative analysis of the visualization preferences sought by AML decision makers, highlighting the role of tailored visualization techniques in AML investigation.

By analyzing the AML users' distinct needs, we gain a comprehensive understanding of the challenges that AML investigators encounter in their work. This examination offers a nuanced perspective on the visualization requirements specific to the AML context and potential avenues for enhancing the efficacy of visualization tools for these professionals.

As mentioned in section \ref{construtivevis}, \citet{Dimara2021Unmet} recommended four types of visualization tools to support decision makers: \textit{flexible interface}, \textit{interrogator tools}, \textit{scenario-based simulations}, and \textit{trade-off overviews}. Specifically within flexible interface, the system created could make use of four approaches to improve the flexibility, including \textit{social actions}, \textit{input data actions}, \textit{mapping and presentation actions}, \textit{processing} and \textit{interaction mean} \cite{Dimara2021Unmet}. In addition to those approaches, this research also employed \citet{constructive}'s \textit{constructive visualization} theory to create an interface that allows the decision makers to construct their own visualization to perform AML investigation. 

\subsubsection{Flexible interface}\hfill\\
This section delves into how to design a versatile and integrated system that supports AML decision makers through the use of \textit{social actions}, \textit{mapping and presentation actions}, \textit{processing} and \textit{interaction mean}. 

\textbf{Facilitate social actions}\hfill\\
Through the interviews, workshops and usability evaluation, it is found that the option to collaborate and share insights between AML users holds a significant importance. Currently, if a user wants to share info about an alert with someone else, that person has to redo the entire investigation, wasting time and effort. This prevents users from benefiting from previous investigations and leads to duplication.

To address this, the new interface proposed a solution for the users to share the investigation as a link or an Excel files, allow easy sharing and collaboration. In the next design iteration, users can also utilize the insights from previous investigation by having an overview of the previous alert and getting actionable insights. By doing so, we aim to design a flexible interface that cuts down on duplicated effort, encourages collaboration, and lets AML investigators learn from each other's work for more efficient decision making.

\textbf{Mapping and presentation actions}\hfill\\
\citet{Dimara2021Unmet} indicated that decision makers consistently expressed a preference for specialized representations such as flow charts, bullet lists, decision trees, and action-focused formats.  Recognizing the value of these formats in enhancing decision making efficiency, the study explored their integration within the interface. 

During the prototype development phase, several action-focused formats were considered. One such notion involved the incorporation of a checklist of criteria, designed to support decision tasks. The objective of this feature was to provide decision makers with a structured approach to guide their decision making process. However, technical constraints and the complexity of the current system, coupled with the project's scope, led to the omission of this checklist during the definition phase.

Another concept explored was the visualization of user actions in the form of tabs, mirroring distinct steps within the decision flow. This approach aimed to provide a clear and navigable structure for users to engage with. In response to this idea, the prototype was implemented to feature tabs, each representing a sequential step in the decision making process. However, during usability testing, an interesting observation emerged. Users appeared to be less aware of the tab-based representation as indicative of their workflow progression. The tabs' role as markers for decision steps seemed to elude some users, indicating the need for further refinement in communicating the concept.

To address this observation, future iterations of the design can focus on enhancing the visibility and intuitiveness of action-focused formats. By refining the visual cues and user prompts associated with these formats, the interface can more effectively guide decision makers through their workflows. This might involve clearer labeling, interactive cues, or visual highlights that accentuate the tab-based navigation's significance. 

% \ref{fig:Lofi-user-flow}
% Need for using payment method to identify shopper behavior
% Need for payment list 

\textbf{Interaction means}\hfill\\
Visualization techniques presents a unique opportunity to expand the set of interaction methods available to users, thereby enriching the overall flexibility of their actions. In the case of AML investigators, there is a strong need for interaction means. The users suggested to incorporate hovering and zooming functions, which allow users to explore visual representation and retrieve additional information. Hovering over data points provides contextual details, aiding comprehension, whereas zooming permits users to explore the graph in details, aiding the identification of relationships and outliers. Another requirement mentioned by AML investigators was the necessity for interactive filters. These filters can be used to exclude specific data points that are not relevant to the current inquiry, thereby enhancing the relevance of the analysis. In addition, geographically-based filters were highlighted by the users, enabling the identification of anomalies and relationships that might be location-specific. By leveraging these interaction means, the new visualization tool empower users with the ability to navigate through complex data and uncover more meaningful data that that might remain concealed in more static approaches.

\textbf{Processing}\hfill\\
Another approach proposed by \citet{Dimara2021Unmet} to increase interface flexibility is guiding decision makers in articulating their requirements when handling extensive data processing tasks. The usability testing  shed light on the significant value that explanation and contextual guidance can bring to the decisions making process. The findings suggest that explanations help bridge the gap between the complex data representation and the user's comprehension, offering insights into the meaning and significance of visual cues. However, the new tool still lacks processing-driven features. In the next iteration, the visualization tool could be designed more toward a personalized decision support system. For example, AML investigators can interact with the system, request clarifications on visual encodings, and receive contextual guidance tailored to their goals.

\subsubsection{Interrogator tools for Intelligence phase}\hfill\\
Interrogator tools, as mentioned in section \ref{construtivevis}, represent a valuable approach to aiding decision makers in the Intelligence phase of the decision making process. These interrogator play a crucial role in assisting users to effectively define the questions they should be asking. To achieve this, these tools need to address two key aspects: 1) enabling users to flexibly store, organize, and annotate both quantitative and qualitative data, and 2) providing a user-friendly, iterative mechanism for scanning, aligning, and recombine different forms of information \cite{Dimara2021Unmet}.

The concept of user discretion in data handling was incorporated into the prototype by incorporating a star icon. This star icon functionality allowed users to store, organize, and annotate information as they progressed through their investigation. Meanwhile, the second aspect was realized through the integration of an overview right sidebar. This feature enabled users to swiftly scan information and explore various combinations of data while simultaneously interacting with the graph displayed on the left side of the interface (figure \ref{fig:Hifi-graph-overview}).

The usability testing of the prototype showed that the automated graph served as a valuable tool for scoping the investigation. Users found the automated graphs to be particularly beneficial in helping them understand the scope of their inquiries. However, it was noted that the manual graph builder, while potentially advantageous when users had a clear idea of what to seek, wasn't always the case that the user would know exactly what to find. This observation indicated that the manual graph builder was perceived more as a tool for validation rather than a interrogator tool. As a result, the findings suggest that the users would tend to turn to the manual graph builder when they had a hypothesis to validate, and use the automated flow for question formulation.

\subsubsection{Constructive visualization for Design phase}\hfill\\
After decision makers gather insights about a problem from the Intelligence phase, they move towards evaluating potential solutions during the \textit{design phase} (see section \ref{decision task}). The research proposed that constructive visualization could provide support to aid decision makers in this crucial phase. They can simulate various scenarios by altering parameters, variables, or conditions, and observe how the visualizations change in response. By visualizing behaviors of shoppers across different time periods, geographical locations, and stores, decision makers are enabled to conduct a comparative analysis. In their process of adjusting parameters, relationships, and variables to explore a spectrum of visualization alternatives, decision makers could attain a more comprehensive understanding of the subject matter under scrutiny, therefore aiding in the assessment of associated risks.

This research employed \citet{constructive}'s \textit{constructive visualization} theory to create a prototype that allowed the decision makers to construct their own visualization to perform AML investigation.  As mentioned in section \ref{construtivevis}, constructive visualization has three advantages. Firstly, it allows users to create their own visualizations, promoting engagement and understanding. Secondly, it enables sharing of these visualizations, fostering knowledge exchange. Thirdly, it encourages discussion and collaboration, leading to more thorough analyses and insights. Therefore, the prototype was developed to embody these principles allows users to create custom visualizations. 

Firstly, AML users can leverage a customized query feature located in the prototype's sidebar to craft visualizations tailored to their specific requirements. Additionally, users can employ their own rule-based custom queries to delve deeper into the data (see \ref{fig:Hifi-graph-builder}). Secondly, the prototype enabled users to share their created visualizations to make them available for other analysts to explore and learn from. Additionally, users could save notes to their investigation, providing context and insights that can be accessed by others. Although the feature for discussion is not yet integrated, it remains a promising feature for future iterations.

Interestingly, usability testing revealed differential preferences among various user types (AML first-line analysts, quality controllers, and compliance officers) regarding this visualization approach. Among them, compliance officers exhibited the highest usability scores and satisfaction levels. Their extensive experience and pivotal role as ultimate decision makers in assessing the legitimacy of suspicious alerts suggest a heightened need for data exploration and flexible visualization tools. This finding underscores the significance of user-centric visualization tools, particularly for those with different analytical responsibilities and domain expertise.

\subsubsection{Trade-off overviews of Choice phase}\hfill\\
As indicated in section \ref{construtivevis}, \citet{Dimara2021Unmet} suggested using trade-off overviews, such as multi-attribute choice tasks to define the importance of decision criteria and visually combine multiple attributes into aggregated scores. This approach presented potential in aiding decision makers by providing a structured framework for decision assessment. However, the interactions with the end-users revealed that the primary challenges in their workflow did not stem from a lack of aggregated scores for decision making. Instead, their concerns predominantly revolved around the inefficiencies within the system for data collection and comparison. Therefore, the design focus was redirected towards developing solutions tailored to the Intelligence and Design phases of the decision making process, where the identified pain points were more prominent.

Furthermore, discussions with the AML product manager emphasized a relatively lower priority for this specific feature. The organization's pressing need was to streamline the data gathering process and enhance data comparison efficiency. While the concept of aggregating multiple attributes into scores garnered positive feedback from the team, its implementation was not deemed an immediate priority due to the organization's strategic emphasis on expediting data collection. Nonetheless, the notion of incorporating aggregated scores to aid decision making remains well-received and may serve as a potential solution for exploration in future iterations.

\newpage
\section{CONCLUSION}\label{section-conclusion}
%The conclusion section summarizes the key findings, reiterates the significance of the research, and draws conclusions based on the evidence presented. It may also discuss the practical implications and potential applications of the research.
In this research, a new visualization tool was designed to support the decision making process of AML investigators. To address this, the following research question was proposed: 
\begin{quote}
\textit{How can information visualization be employed to enhance the decision making process for Anti Money laundering in financial organization?}
\end{quote}
To answer this question, the study employed the Double Diamond design process, which includes Discover, Define, Develop, and Delivery phase. In the Discover phase, we tapped into the critical decision method to uncover the challenges faced by AML investigators and identify the crucial points where decisions come into play. Moving forward, the Define phase employed user journey mapping to chart out how users interact with the tool at each step. While the user journey mapping focuses on understanding user interactions, requirement engineering goes deeper to identify specific functionalities and features the system needs. In the Develop phase, the Creative Problem Solving workshop proved pivotal in sparking diverse ideas for the tool's design. These ideas underwent several evaluation, serving as the inspiration for our initial prototype. Starting from the sketches generated during the workshop, a low-fidelity prototype was crafted, which was further refined through iterative feedback cycles. Through multiple rounds of feedback, a final prototype was created. In the Delivery phase, the prototype was evaluated with the end users utilizing techniques like think-aloud method, system usability scale and post-test interviews. 

\subsection{Main findings}
The result of our study is a powerful visualization tool that effectively addresses complex challenges in AML investigations while highlighting the importance of structured design methodologies. Our research combines insights from AML investigators, design frameworks, and user-centered evaluations, significantly contributing to the evolution of decision making tools within financial organizations. The study revealed the following important findings:

The AML decision making process involves three key user personas: first line analysts, second line compliance officers, and quality controllers. While these users have the same goal to determine the legitimacy of an alert and mitigate risk, these personas exhibit distinct approaches, expertise levels, and responsibilities. First line analysts, typically early in their careers, require validation from second line and quality control. Quality controllers play a crucial role in verifying the accuracy of the work carried out by first line analysts, while compliance officers, who has higher seniority, is the decision makers who make the ultimate judgments on the legitimacy of alerts and frequently collaborate with the authorities

The in-depth interviews conducted during the study revealed several recurring challenges in the user workflow. Deficiencies in documentation, sense-making difficulties, communication gaps, tedious data gathering, tool inflexibility, and insufficient collaboration rituals were identified as major obstacles to effective decision making. To address these challenges, the interviewees offered several recommendations for the design of an improved tool. These recommendations revolve around enhancing the existing graph network visualization, prioritizing automation and quick information retrieval, facilitating efficient note-taking, and offering an intuitive overview of quantitative data. 

This study builds on previous research by \citet{Dimara2021Unmet} (see section \ref{decisionneeds}) to identify key needs of decision makers, including \textit{explanation of analyses}, \textit{information reduction} and \textit{qualitative analysis}. However, the study goes further by introducing a new concept of the \textit{need for placing data within broader contexts}. The findings show that AML users prioritize qualitative analysis and explanation of analyses, consistent with \citet{Dimara2021Unmet}'s research. However, the study also reveals that AML users place less emphasis on information reduction while emphasizing the importance of contextualizing data.

Furthermore, the study's findings revealed that users positively embraced the concepts of a \textit{flexible interface} and \textit{interrogator tools}. The flexible interface encompassed design elements that support social action, mapping and presenting of actions, interaction means, and data processing. Users also were also keen on interrogator tools that help them formulate relevant questions. 

Additionally, the response to the \textit{constructive visualization} concept was varied among users, with mixed reactions stemming from the usability evaluation. While first line analysts and quality controllers face challenges with this approach, compliance officers with decision making authority show higher levels of usability and satisfaction.

\subsection{Limitations}
While the study provided several positive contributions for the development of a new visualization tool, several limitations should be acknowledged.

One major limitation was the time constraints of the research. Due to time limitations, the study was unable to fully realize the envisioned development of the new visualization tool through coding. Although the intention was to create the tool using the Svelte framework, the prototype was solely realized within the Figma due to these constraints. Consequently, certain interactive features of the graph visualization, such as zooming and node manipulation, were restricted. Recognizing this limitation, efforts were directed towards maximizing the available interactions within the prototype. Currently, the prototype is being adopted by the company's development team for further utilization.

Another downside factor regarding the current methodology is the limitation in the evaluation of user performance due to the lack of quantitative metrics. The ideal study design would have included a quantitative comparison of task completion times using both the old and new tools. However, the interactive prototype's limitations made it difficult to obtain robust quantitative measurements. Therefore, the evaluation focused on users' subjective experiences and insights, providing valuable depth of understanding but restricting a comprehensive assessment of performance improvements. Future endeavors in this domain should strive to integrate both qualitative and quantitative methodologies to provide a more holistic evaluation of user performance and tool efficacy.

\subsection{Recommendations for future research}
The current study provides ample opportunities for further research that can extend its findings. 

To achieve this, further work could be done with more financial organizations. Although the study used real life use cases within a large financial organization, other financial organizations could have different processes different tools, therefore they may have different challenges and needs. The visualization tool should also be tailored to different contexts to uncover unique challenges and refine its adaptability across the industry. 

To evaluate user task performance, more quantitative measurements should be introduced, while integrating graph analytics could unlock additional layers of insights that will maximize the tool's analytical potential. 

To enhance decision making support, future iterations could focus on providing comprehensive trade-off overviews and aggregating multiple attributes into informative scores.  This focus in the Choice phase could empower decision makers with more nuanced insights, enhancing their ability to navigate complex decisions effectively. In the next iteration, the visualization tool could also be designed more toward a personalized decision support system. For example, AML investigators can interact more with the system, request clarifications on visual encodings, and receive contextual guidance tailored to their goals. In addition, introducing a platform for user discussion could further encourage collaboration and knowledge sharing among investigators. 

As research evolves, these directions promise to refine the tool's efficacy in the dynamic context of financial organizations, ultimately leading to a more effective decision support system.

%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
\newpage
\bibliographystyle{ACM-Reference-Format}
\bibliography{bibliography}

\appendix
\onecolumn
\section{List of Abbreviations}\label{abbreviations}
\begin{center}
\begin{tabular}{l l}
\textbf{Abbreviation} & \textbf{Description} \\
\hline
AML & Anti Money Laundering \\
AI & Artificial Intelligence \\
ML & Machine learning \\
MoSCoW & “must-have” “should-have” “could-have” and “won't-have" \\
InfoVis & Information Visualization \\
OSINT & Open Source Intelligence \\
SUS & System Usability Scale \\
QOC & Questions, Options, Criteria 
\end{tabular}
\end{center}

\section{Discover phase}\label{discovery}
% \newpage
\begin{figure}[h]
     \centering
     \includegraphics[width=1\columnwidth]{figures/Data Collection Procedure.png}
     \caption{An overview of the questions being asked in the semi-structured interviews}
\end{figure}

\newpage
\section{Define phase}\label{define}
\begin{table}[h]
\centering
\resizebox{0.7\textwidth}{!}{
\footnotesize
\begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}p{0.8cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}p{1cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}p{1.5cm}}
\toprule
\textbf{Epic ID} & \textbf{Epics} & \textbf{Story ID} & \textbf{User Stories} & \textbf{Priority} \\
\midrule
E1 & As a first line analyst, I want to analyze the alerts generated by the automated detection method so that I can make sure the alerts are accurate & U1 & As a first line analyst, I want to have more contextual information on the alert so that I understand why the alert is generated & Must \\
& & U2 & As a first line analyst, I want to have more contextual information on the merchants so that I can find risk mitigating factors & Could \\
& & U3 & As a first line analyst, I want to have more contextual information on the sub-merchants so that I can find risk mitigating factors & Could \\
& & U4 & As a first line analyst, I want to have more contextual information on the shoppers so that I can find risk mitigating factors & Should \\
\midrule
E2 & As a first line analyst, I want to communicate my assessment to other analysts so that I can also make use of other analysts’ assessment for similar alerts in the future & U5 & As a first line analyst, I want to export my investigation so that I can share the result with other stakeholders & Could \\
& & U6 & As a first line analyst, I want to have documentation of all the investigation steps so that I can make sure my investigation is reliable and accurate & Could \\
\bottomrule
\end{tabularx}
}
\caption{An overview of the user stories from first line analysts}
\label{tab:US-1}
\end{table}

\begin{table}[h]
\centering
\resizebox{0.66\textwidth}{!}{
\footnotesize
\begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}p{0.8cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}p{0.8cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}p{1cm}}
\toprule
\textbf{Epic ID} & \textbf{Epics} & \textbf{Story ID} & \textbf{User Stories} & \textbf{Priority} \\
\midrule
E3 & As a compliance officer and quality controller, I want to review the work of first line analysts thoroughly so that I can make sure that their investigation is accurate & U7 & As a compliance officer, I want to have all previous investigation on the alert presented to me so that I can review them & Should \\
& & U8 & As a compliance officer, I want to have all previous investigation on the sub-merchants so that I can review them & Should \\
& & U9 & As a compliance officer, I want to have all previous investigation on the shoppers so that I can review them & Should \\
\midrule
E4 & As a compliance officer, I want to report my assessment to the authorities and other analysts so that I can take action on suspicious activities & U10 & As a compliance officer, I want to export my investigation so that I can share the result with other stakeholders & Could \\
& & U11 & As a compliance officer, I want to have documentation of all the investigation steps so that I can make sure my investigation is reliable and accurate & Could \\
\bottomrule
\end{tabularx}
}
\caption{An overview of the user stories from compliance officer and quality controller}
\label{tab:US-2}
\end{table}

\begin{table}[h]
  \centering
  \resizebox{0.66\textwidth}{!}{
  \footnotesize
  \begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}p{0.8cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}p{0.8cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}p{1cm}}
  \toprule
    \textbf{Epic ID} & \textbf{Epics} & \textbf{Story ID} & \textbf{User Stories} & \textbf{Priority} \\
    \midrule
    E5 & As a quality controller, I want to communicate my assessment to other analysts so that I can improve my workflow & U12 & As a quality controller, I want to communicate my assessment to other analysts so the first line analysts could improve their investigation based on my suggestions & Won't \\
    & & U13 & As a quality controller, I want to have a collaborate tool with other analysts so that I can work with multiple people at the same time & Won't \\
    \bottomrule
  \end{tabularx}
  }
  \caption{An overview of the user stories from quality controller}
  \label{tab:US-3}
\end{table}

\newpage
\begin{table}[htbp]
  \centering
  \resizebox{0.66\textwidth}{!}{
  \footnotesize
    \begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}p{0.8cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}p{0.8cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}p{1cm}}
      \toprule
      \textbf{Epic ID} & \textbf{Epics} & \textbf{Story ID} & \textbf{User Stories} & \textbf{Priority} \\
      \midrule
      E6 & As a compliance officer, first line analyst and quality controller, I want to reduce the time to gather data from multiple sources so that I can find valuable information to help me make a decision about the investigation & U14 & As a compliance officer, first line analyst and quality controller, I want to have aggregated information on a merchant so that I can have more contextual information for my investigation & Must \\
      & & U15 & As a compliance officer, first line analyst and quality controller, I want to have aggregated information on a shopper so that I can have more contextual information for my investigation & Must \\
      & & U16 & As a compliance officer, first line analyst and quality controller, I want to be able to search and filter identifiers/nodes so that I can access information quicker & Must \\
      & & U17 & As a compliance officer, first line analyst and quality controller, I want to spend as little time on navigation as possible so that I can focus on my analysis & Should \\
      E7 & As a compliance officer, first line analyst and quality controller, I want to see patterns in data so that I can capture unusual behaviors from the shoppers and sub-merchants & U18 & As a compliance officer, first line analyst and quality controller, I want to see the interactive connection between customers and shoppers so that I can get more information about their behaviors & Must \\
      & & U19 & As a compliance officer, first line analyst and quality controller, I want to have a visualization of complex data so that I can detect the expected and discover the unexpected behaviors & Must \\
      & & U20 & As a compliance officer, first line analyst and quality controller, I want to see transaction data of a shopper so that I can understand the shopper behaviors & Must \\
      & & U21 & As a compliance officer, first line analyst and quality controller, I want to see the timeline of shopper behaviors so that I can understand the shopper behaviors & Must \\
      E8 & As a compliance officer, first line analyst and quality controller, I want to have the flexibility to aggregate data myself so that I can generate an assessment about the investigation & U22 & As a compliance officer, first line analyst and quality controller, I want to create my own query so that I can customize my analysis & Should \\
      & & U23 & As a compliance officer, first line analyst and quality controller, I want to save a query so that I can reuse them for my analysis & Should \\
      & & U24 & As a compliance officer, first line analyst and quality controller, I want to cluster similar alerts based on my criteria so that I can find a suspicious group & Could \\
      E9 & As a compliance officer, first line analyst and quality controller, I want to judge between multiple criteria so that I can make a decision about the case & U25 & As a compliance officer, first line analyst and quality controller, I want to have a risk score on a shopper so that I can evaluate the risk factors of this shopper & Should \\
      & & U26 & As a compliance officer, first line analyst and quality controller, I want to have an explanation of how the system links different accounts so that I can trust the system is providing me accurate information & Should \\
      & & U27 & As a compliance officer, first line analyst and quality controller, I want to save my analysis to my note so that I can use them to evaluate my decision & Must \\
      & & U28 & As a compliance officer, first line analyst and quality controller, I want to have a checklist for investigation criteria so that I can make sure I do not miss any important information & Must \\
      & & U29 & As a compliance officer, first line analyst and quality controller, I want to have an aggregated score for the evaluation criteria so that I can make sure my decision is objective & Could \\
      \bottomrule
    \end{tabularx}
    }
  \caption{An overview of the user stories from all user personas}
  \label{tab:US-4}
\end{table}

\newpage
\section{Develop phase}\label{develop}
\subsection{Problem scenarios for CPS workshop}\label{case-guide}
\textbf{Introduction}\hfill\\
Usually a red flag is generated by a detection method on the big data platform which is then reviewed by analysts as part of the investigation. During the investigation the analyst will ensure the signal was generated correctly and it was inline with the relevant unusual behaviour defined in the scenario. For the purpose of these exercises we will use red flags as the term referring to something that indicates unusual behaviour and must be reviewed and checked by the analyst. Please assume that the red flags have already been generated!
Red Flags need to be checked and reviewed but also need to be contextualised to a customers overall transaction profile and also other unrelated shopper behaviours.

\textbf{Summary of investigation steps (high level):}
\begin{enumerate}
    \item Review the links between transactions or internal customers and ensure they make sense
    \item Assess the relative money laundering risk (red flags)
    \item Record analysis and decision
\end{enumerate}

\textbf{Action}
\begin{quote}
    Create investigation tool which assists the investigation and solves some of the challenges listed in the “challenges section”.
\end{quote}
\textbf{Case 1}\hfill\\
The company processes for many reputable customers which sell items of considerable value. Money launderers will re-integrate cleaned-illicit-funds into the financial system by purchasing High Value Goods which hold significant value. Typically shopper transaction histories will be largely made up of transactions at one or many customers selling High Value Goods.

Red Flags
\begin{itemize}
    \item Individual high amount (payin) from single shopper
    \item High velocity of between multiple payins (multiple payins)
    \item Evidence of repetition of transactions
    \item The shopper is sanctioned, is a Politically exposed person (high risk of corruption)
\end{itemize}

\textbf{Case 2}\hfill\\
The same group of shoppers have been identified across multiple account holders using platforms. This is indicates a classic customer shopper collusion case whereby money laundering gangs are attempting to legitimize their funds by using multiple shoppers to generate purchases for phoney products. Subsequently “cleaned” funds are paid out to the account holders bank account.

Red Flags
\begin{itemize}
    \item Overlapping KYC identifiers between account holders and shoppers
    \item Overlapping shopper identifiers across multiple accounts holders
    \item Group of shoppers make abnormally large portion of an account holders total processing
    \item Periodic repetitive transactions (payins) from identified group
\end{itemize}

\textbf{Case 3}\hfill\\
Many small incoming transfers are entering a balance account of which are then immediately transferred to a bank account in a different geographic location. Note that incoming transfers can be incoming bank transfers or acquiring payins whilst the payout will always be an ongoing bank transfer.

Red Flags
% \begin{itemize}
%     \item High velocity incoming and outgoing transactions
%     \item Shoppers/senders are sending repetitive payins/bank transfers
%     \item Mismatch between account holder bank account and recipient bank account
% \end{itemize}

% \subsection{CPS workshop results}
% \begin{figure}[h]
%      \centering
%      \includegraphics[width=1\columnwidth]{figures/AML workshop copy.png}
%      \caption{The sketches made by the participants during the Creative Problem Solving workshop}
%       \label{fig:workshop-sketch}
%  \end{figure}

% \begin{figure}[h]
%       \centering
%       \includegraphics[width=1\columnwidth]{figures/Rapid prototype.png}
%       \caption{An overview of the low fidelity prototype}
%       \label{fig:rapid-prototype}
% \end{figure}

% \newpage
% \section{Delivery phase}\label{deliver}
% \subsection{Usability evaluation protocol}
% \begin{figure}[h]
%   \centering
%   \includesvg[width=1\textwidth]{Usability test/Usability test design.svg}
%   \caption{An overview of the usability evaluation procedure}
%   \label{fig:usability-test-design}
% \end{figure}

% \begin{figure}[h]
%       \centering
%       \includegraphics[width=0.7\columnwidth]{figures/Consent.png}
%       \caption{An overview of consent form being sent to the participants}
%       \label{fig:consent-form}
% \end{figure}

% \subsection{Usability evaluation coding observations}
% \begin{figure}[h]
%       \centering
%       \includegraphics[width=1\columnwidth]{Usability test/Condens.png}
%       \caption{An overview of codes generated}
%       \label{fig:condens-code}
% \end{figure}

% \begin{figure}[h]
%      \centering
%      \includegraphics[width=0.6\columnwidth]{figures/Tag groups categorized by the number of participants.png}
%      \caption{Tag groups categorized by the number of participants}
%      \label{fig:tag-group-participant}
% \end{figure}

% \begin{figure}[h]
%      \centering
%      \includegraphics[width=1\columnwidth]{figures/Participant-excerpts.png}
%      \caption{An overview of the observation notes categorized by the participants and the level of usability issues}
%      \label{fig:participant-excerpts}
% \end{figure}

% \begin{figure}[h]
%      \centering
%      \includegraphics[width=1\textwidth]{Usability test/Category-excerpt-table.png}
%      \caption{Category excerpt table}
%      \label{fig:Category-excerpt-table}
% \end{figure}

\end{document}
\endinput
%%
%% End of file `sample-authordraft.tex'.


==> section3.tex <==
\section{Discussion and Future Work}

blah blah\\\\

\section{Conclusion}

THE END\\\\\\
